Are Proactive Interventions for Reddit Communities Feasible?

Reddit has found its communities playing a prominent role in originating and propagating problematic socio-political discourse. Reddit administrators have generally struggled to prevent or contain such discourse for several reasons including: (1) the inability for a handful of human administrators to track and react to millions of posts and comments per day and (2) fear of backlash as a consequence of administrative decisions to ban or quarantine hateful communities. Consequently, administrative actions (community bans and quarantines) are often taken only when problematic discourse within a community spills over into the real world with serious consequences. In this paper, we investigate the feasibility of deploying tools to proactively identify problematic communities on Reddit. Proactive identification strategies show promise for three reasons: (1) they have potential to reduce the manual efforts required to track communities for problematic content, (2) they give administrators a scientific rationale to back their decisions and interventions, and (3) they facilitate early and more nuanced interventions (than banning or quarantining) to mitigate problematic discourse.

==> Makefile <==
# Makefile for LaTeX files

# Original Makefile from http://www.math.psu.edu/elkin/math/497a/Makefile

# Please check http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile
# for new versions.

# Copyright (c) 2005,2006 (in order of appearance):
#	Matti Airas <Matti.Airas@hut.fi>
# 	Rainer Jung
#	Antoine Chambert-Loir
#	Timo Kiravuo

# Permission is hereby granted, free of charge, to any person obtaining
# a copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to
# permit persons to whom the Software is furnished to do so, subject to
# the following conditions: 

# The above copyright notice and this permission notice shall be
# included in all copies or substantial portions of the Software. 

# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND,
# EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.
# IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY
# CLAIM, DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT,
# TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE
# SOFTWARE OR THE USE OR OTHER DEALINGS IN THE SOFTWARE. 

# $Id: Makefile,v 1.18 2006-06-19 10:58:11 mairas Exp $

LATEX	= pdflatex
BIBTEX	= bibtex
MAKEINDEX = makeindex
XDVI	= xdvi -gamma 4
DVIPS	= dvips
DVIPDF  = dvipdft
L2H	= latex2html
GH	= gv

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"

DATE=$(shell date +%Y-%m-%d)

COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false

# These are OK

SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
TRG	= $(SRC:%.tex=%.dvi)
PSF	= $(SRC:%.tex=%.ps)
PDF	= $(SRC:%.tex=%.pdf)

# These are not

#BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))
#DEP     := $(shell perl -ne '($$_)=/^[^%]*\\include\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $(SRC))
#EPSPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $(SRC) $(DEP))


define run-latex
	$(COPY);$(LATEX) $<
	egrep $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) >/dev/null; true
	egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	$(RM) $(<:%.tex=%.toc.bak)
	# Display relevant warnings
	egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef

define run-pdflatex
	LATEX=pdflatex
	@$(run-latex)
endef

define get_dependencies
	deps=`perl -ne '($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $<`
endef

define getbibs
	bibs=`perl -ne '($$_)=/^[^%]*\\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $< $$deps`
endef

define geteps
	epses=`perl -ne '@foo=/^[^%]*\\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $< $$deps`
endef

define manconf
	mandeps=`if test -r $(basename $@).cnf ; then cat $(basename $@).cnf |tr -d '\n\r' ; fi`
endef

all 	: $(TRG)

.PHONY	: all show clean ps pdf showps veryclean

clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.dvi=%.aux) $(TRG:%.dvi=%.bbl) $(TRG:%.dvi=%.blg) $(TRG:%.dvi=%.log) $(TRG:%.dvi=%.out) $(TRG:%.dvi=%.idx) $(TRG:%.dvi=%.ilg) $(TRG:%.dvi=%.ind) $(TRG:%.dvi=%.toc) $(TRG:%.dvi=%.d)

veryclean	: clean
	  -rm -f *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind *.ps  *~

# This is a rule to generate a file of prerequisites for a given .tex file
%.d	: %.tex
	$(get_dependencies) ; echo $$deps ; \
	$(getbibs) ; echo $$bibs ; \
	$(manconf) ; echo  $$mandeps  ;\
	echo "$*.dvi $@ : $< $$deps $$bibs $$epses $$mandeps" > $@ 

include $(SRC:.tex=.d)

# $(DEP) $(EPSPICS) $(BIBFILE)
$(TRG)	: %.dvi : %.tex
	  @$(run-latex)

$(PSF)	: %.ps : %.dvi
	  @$(DVIPS) $< -o $@

#$(PDF)  : %.pdf : %.dvi
#	  @$(DVIPDF) -o $@ $<
# To use pdflatex, comment the two lines above and uncomment the lines below
#$(PDF) : %.pdf : %.tex
#	@$(run-pdflatex)


show	: $(TRG)
	  @for i in $(TRG) ; do $(XDVI) $$i & done

showps	: $(PSF)
	  @for i in $(PSF) ; do $(GH) $$i & done

ps	: $(PSF) 

pdf	: $(PDF) 

# TODO: This probably needs fixing
html	: @$(DEP) $(EPSPICS)
	  @$(L2H) $(SRC)



######################################################################
# Define rules for EPS source files.

# These rules probably just cause unnecessary confusion, so commenting
# them away for the time being. -- mairas 2005-01-12

#%.eps: %.sxd
#	$(OUTDATED)
#%.eps: %.sda
#	$(OUTDATED)
#%.eps: %.png
#	$(OUTDATED)
#%.eps: %.sxc
#	$(OUTDATED)
#%.eps: %.xcf
#	$(OUTDATED)
#%.eps: %.zargo
#	$(OUTDATED)
#%.eps: %.m
#	@egrep -q $(MPRINT) $< && ($(OUTDATED))


==> conclusions.tex <==
\section{Conclusions}\label{sec:conclusions}

Reddit employs a small number of human administrators
\cite{We-are-the-nerds} to set site-wide policy and identify violating
communities. In addition to the growing size of the platform, our analysis in
\Cref{sec:evolution} show subreddits may not converge to vocabulary and user
stability suggesting a need for constant moderation making human-only
administration prohibitively expensive. This results in administrators relying
on user generated and media reports of egregious violations as we show in
\Cref{sec:predictors:results:features}. This reactive approach has limited
success and leads to delayed interventions. As shown in previous research,
timely interventions are key to mitigating hate speech and maintaining civility
on the platform. Alternative to the current reactive approach, we propose an
automated proactive approach designed to aid administrators focus their efforts
and reveal hidden problematic subreddits.

In \Cref{sec:evolution:results} we observe that the evolutionary characteristics
of problematic subreddits is different from non-problematic subreddits. This
suggests opportunities for training a classifier to predict problematic
subreddits proactively. We exploit these differences in evolutionary
characteristics to build simple, explainable, and accurate machine learning
models to characterize the current and predict the future behavior of different
communities.  To use our model in real world, we design a continual learning
pipeline enabling our model to indirectly learn changes made to the content
policy.

The non-static nature of Reddits content policy requires
retraining the model to learn novel administrative decisions. Furthermore, the
nature of autonomous predictive policing systems make them susceptible to bias.
Therefore, we recommend using such tools to assist human moderators by
emphasizing communities that may pose a future threat and consequently require
special attention.



==> moderation.tex <==
\section{Impact of Interventions}\label{sec:moderation}

So far our results have shown that topics and user bases associated with
subreddits, on average, are constantly evolving (\Cref{sec:evolution}) and
the characteristics of this evolution can be used to perform early
identification of problematic subreddits (\Cref{sec:predictors}). These
findings suggest that proactive community administration and moderation
interventions can be used to mitigate the impact of such communities. In this
section, we focus on understanding the impact of current administrative
interventions (\ie bans and quarantines) on communities classified as
problematic by Reddit administrators. Specifically, we test: \textbf{H3.
Subreddit ban and quarantine interventions, as currently performed by Reddit
administrators, do not reduce problematic behavior on Reddit}. These hypotheses,
if valid, will suggest the need for new intervention design or deployment
strategies. If invalid, it will suggest that current interventions are
sufficient for the platform. Our methodological and result contributions are
highlighted in \Cref{tab:moderation}.

\begin{table}
  \centering
  \small
  \begin{tabular}{ll}
    \toprule
    \textbf{Methodological questions} & \textbf{\Cref{sec:moderation:methods}}\\
    \midrule
    How do we quantify the quantity and quality of user participation? & \Cref{sec:moderation:methods:user-behavior}\\
    How do we quantify the impact of events on user participation? & \Cref{sec:moderation:methods:interventions}\\
    \midrule
    \textbf{Research questions} & \textbf{\Cref{sec:moderation:results}}\\
    \midrule
    What is the impact of joining a problematic community on user behavior? & \Cref{sec:moderation:results:joining}\\
    What is the impact of interventions on problematic communities on user behavior? & \Cref{sec:moderation:results:intervention}\\
    \bottomrule
  \end{tabular}
  \caption{Hypothesis 3: Subreddit ban and quarantine interventions, as
  currently performed by Reddit administrators, do not reduce problematic
  behavior on Reddit. Summary of methods and results.}
  %\vspace{.2in}
  \label{tab:moderation}
\end{table}
 
\para{High-level overview.} At a high-level, our goal is to quantify the change
in user behavior, in the broader community, that occurs as a result of two
types of events: (1) joining a subreddit later classified as problematic and
(2) administrator interventions (\ie bans and quarantines) on subreddits
categorized as problematic. To achieve this goal, we need to develop
methods to (1) quantify user behavior and (2) measure the impact of each of the
above events on these metrics. We accomplish this using the following approach,
which is explained in more detail in \Cref{sec:moderation:methods}. 
First, we quantify user behavior using two metrics -- incidence of hateful
commenting activity and quantity of participation in communities later
classified as problematic by Reddit administrators. Second, to understand the
impact of certain events on their behavior, we carefully select treatment
(users impacted by the event) and control (users similar to treatment group but
not impacted by the event) groups and analyze how their behaviour varies before
and after the joining or intervention event. Using this approach, we find that
current interventions and their application do not result in improved user
behavior or reduce their participation in communities later deemed as
problematic. This validates our hypothesis. Detailed results are presented in
\Cref{sec:moderation:results}.

\subsection{Methods} \label{sec:moderation:methods}

% Our approach for testing the proposed hypothesis requires two main methods.
% First, in \Cref{sec:moderation:methods:user-behavior}, we quantify user
% behavior using two metrics -- incidence of offensive comments and quantity of
% participation in known hateful and dangerous communities. Second, in
% \Cref{sec:moderation:methods:interventions}, to understand the impact of
% certain events on their behavior, we carefully select treatment (users impacted
% by the event) and control (users similar to control group but not impacted by
% the event) groups and analyze how their behaviour varies before and after the
% event.
% 
% First, we need to develop metrics to quantify user behavior
% (\Cref{sec:moderation:methods:user-behavior}). Next, we need to determine how
% to quantify the impact of an event on user behavior
% (\Cref{sec:moderation:methods:interventions}).

\subsubsection{How do we quantify the nature of user participation?}
\label{sec:moderation:methods:user-behavior}

We quantify user behavior using two different metrics -- (1) the incidence rate
of hateful commenting activity on Reddit and (2) the incidence rate of
participation on communities later categorized as problematic by
administrators. We select these metrics since they can accurately reflect the
effectiveness of administrator interventions at improving the civility of
discourse on Reddit as well as effectively curbing the rise of problematic
content on Reddit. We argue that if the current administrative interventions were
effective at achieving these goals, then we should see users of
intervention-affected subreddits curb the behavior that resulted in the
intervention -- \ie behaviors which were deemed to violate the Reddit content
policy on violent, threatening, and harassing speech (for which we use
incidence rates of hateful comments as a proxy) or any other policy violation
(for which we use participation on future problematic subreddits as a proxy). 

\para{Identifying hateful commenting activity.} In order to determine if a user
comment is hateful or not, we rely on a hate speech classifier (Hate Sonar)
developed by Davidson \etal \cite{hatesonar}. Hate Sonar is specifically built
to differentiate between simply offensive speech and hateful speech and relies
on models built using human-annotated social-media posts -- making it
applicable in the current context. In their evaluation of Hate Sonar, Davidson
\etal found that the model had an F1-score of 90\% and the most common error
involved miscategorizing hate speech as offensive speech. This makes the model
useful for obtaining lower-bounds and trends on the incidence of hate speech as
is required by our work. We use Hate Sonar to quantify the fraction of hateful
comments made by users each month, across the entire platform.

% If administrative interventions are successful at
% reducing hateful commenting activity on the users of impacted subreddits, we
% expect to see the incidence rate of such comments drop after the intervention
% is applied. The absence of this reduction will imply that the interventions, as
% designed and applied by Reddit administrators, do not result in improvements of
% user behavior outside of the problematic subreddit. Further, tracking this
% metric will also allow us to 

\para{Identifying participation in problematic communities.} In addition to
tracking hateful commenting activity of users, we also track their
participation in subreddits that are later deemed as problematic. This is done
by tracking the fraction of their comments, each month, that occur in any of
the $\mathfrak{D}_I$ subreddits. 

% If administrative interventions are successful at reducing
% a user's non-compliance with the Reddit content policy, then we expect to see
% a reduction in their participation in communities which eventually belong in
% $\mathfrak{D}_I$. The absence of this reduction will imply that community-level
% interventions, as designed and applied by Reddit administrators, do not reduce
% user participation in policy-violating subreddits.

% We quantify user behavior using two different metrics -- (1) the incidence rate
% of offensive comments and (2) the fraction of their participation that occurs
% in communities known to be hateful or dangerous. We classify offensive comments
% made by users for each month using hatesonar, an offensive speech classifier
% \cite{hatesonar} which allows us to assign an incidence rate of offensiveness for
% each user for each month. In addition, for each user for each month, we also
% record the fraction of user activity (in terms of comments made) that occurred
% in dangerous ($\mathfrak{D}_B$) and hateful ($\mathfrak{D}_H$) communities.

\subsubsection{How do we quantify the impact of events on user participation?
} \label{sec:moderation:methods:interventions}

We analyze the impact of two types of events on a user's behavior: 
joining subreddit which is eventually place in $\mathfrak{D}_I$ and the banning
or quarantining of a community they participate in. By tracking user behavior
for the months before and after they were impacted by one of these events, we
are able to see general trends which illustrate the impact of the event. We go
one step further in our analysis of the impact of each events -- we compare
user behavior with a control group. This enables us to be more certain about
the attribution of change in trends to the event being studied.

\para{Selection of control group users.} For each user in our treatment group
(\eg user who participated in a $\mathfrak{D}_I$ subreddit), we selected the
user who was not impacted by the corresponding event (\eg did not join the
corresponding problematic subreddit) but shared the most similar participation
behavior. More specifically, we created a participation vector, $v_i$, for
each user, $u_i$, who was active on Reddit during the month of the event, but
not a participant on the studied $\mathfrak{D}_I$ subreddit at any point. The
$j^{th}$ element of $v_i$ corresponds to the number of comments made by $u_i$
on subreddit $s_j$. Next, we used locality sensitive hashing \cite{lsh} to
efficiently identify the approximate nearest neighbors of each treatment user.
We relied on an approximation due to the prohibitive computational expenses
associated with exact neighbor computation for over 2 million treatment users.
Of the candidate approximate nearest neighbors, the euclidean distance metric
was used to identify the neighbor that would serve as the control user. This
process was repeated for every $\mathfrak{D}_I$ subreddit and for each of their
active users. 

\subsection{Results} \label{sec:moderation:results}
% We now focus on understanding the impact of community join
% (\Cref{sec:moderation:results:joining}), ban and quarantine 
% (\Cref{sec:moderation:results:intervention}) events on user behavior. 
% 
\begin{figure*}
	\centering
	\begin{subfigure}[b]{.3\textwidth}
		\includegraphics[width=\textwidth]{H3-new-figs/joining_hate-12.pdf}
		\caption{Metric: Hate speech. \\Event: Joining a $\mathfrak{D}_I$ subreddit.}
		\label{fig:moderation:results:joining:hatespeech}
	\end{subfigure}
	\begin{subfigure}[b]{.3\textwidth}
		\includegraphics[width=\textwidth]{H3-new-figs/DI_ban_participation-12.pdf}
    \caption{Metric: Participation ratio. \\Event: Banning a  $\mathfrak{D}_I$ subreddit.}
		\label{fig:moderation:results:banning:participation}
	\end{subfigure}\qquad
	\begin{subfigure}[b]{.3\textwidth}
		\includegraphics[width=\textwidth]{H3-new-figs/DI_ban_hatespeech-12.pdf}
		\caption{Metric: Hate speech. \\Event: Banning a $\mathfrak{D}_I$ subreddit.}
		\label{fig:moderation:results:banning:hatespeech}
	\end{subfigure}
	\caption{The impact of joining and administrator intervention events on user
  behavior. Month ``0'' represents the month of the event. }
	\label{fig:moderation:results}
\end{figure*}

\subsubsection{What is the impact of joining problematic subreddits on broader
user behavior?}\label{sec:moderation:results:joining}

\Cref{fig:moderation:results:joining:hatespeech} shows the impact of joining
problematic ($\mathfrak{D}_I$) communities on the incidence rates of hateful
comments made by a user. We notice two trends from these results: First, our
treatment users (redditors who eventually joined a $\mathfrak{D}_I$ subreddit)
already have a higher incidence rate than their control user counterparts.
Second, this gets further amplified once they join a problematic community.
Similar results are found when using Hate Sonar to identify offensive comment
incidence rates. This suggests that joining a problematic subreddit does 
negatively impact the platform. 

% We can make several interesting observations from these results. First, we see
% that \emph{joining hateful banned communities increases offensiveness in the broader
% community.} Looking at
% \Cref{fig:moderation:results:joining} we see that during
%  the month of the join event associated with hate subreddits, our treatment
% users show an increase of nearly 2\% in offensive commenting behavior.
% % Interestingly, we see that our treatment users who joined dangerous subreddits
% % show signs of increased 
% % offensiveness from our control group for many months before the join event
% % (\Cref{fig:moderation:results:joining:banned:offensiveness}). Seeking to better
% % understand this trend leads us to our next observation.
% Further, we also see that \emph{hateful communities are a pipeline to
% dangerous communities.} In fact, \Cref{fig:moderation:results:joining}, shows
% that joining  
% a hate community leads to nearly 500\% more activity in dangerous communities.
% Alarmingly, this increase happens within the same month of the join event and
% remains high for many months after. This is strong evidence of a causal
% relationship between joining hate communities and participation in dangerous
% communities. 
% We do not see a similar trend when analyzing the rate of
% participation in hateful communities after joining a dangerous community
% (\Cref{fig:moderation:results:joining:banned:community}).


%\begin{figure}[th]
  %\centering
        %\includegraphics[width=.95\textwidth]{H3-figs/DHBehaviorChangeJoining.png}
    %\caption{The impact of joining hateful communities on user behavior. Month ``0''
    %represents the month of the join event. We show user behavior change in
	%terms of offensive language and participation in dangerous communities.}
  %\vspace{-.15in}
  %\label{fig:moderation:results:joining}
%\end{figure}

\subsubsection{What is the impact of administrator interventions on problematic
subreddits on the behavior of their members?}
\label{sec:moderation:results:intervention}

\Cref{fig:moderation:results:banning:participation} and
\Cref{fig:moderation:results:banning:hatespeech} shows the impact of the
application of community-level bans or quarantines on the participation
behavior of users of problematic subreddits. These results show that current
intervention strategies only result in increased user participation in other
communities which turn problematic. This suggests that users impacted by an
administrative intervention simply continue their problematic activities on
other subreddits rather than moving them off-platform or ceasing such behavior
-- effectively turning effective application of interventions into a game of
whack-a-mole. Further, we also see that there is no reduction in the incidence
rate of hate speech from users of problematic communities after an
intervention.

% quarantining communities on the behavior of their members. We make the
% following observations. First, \emph{bans and quarantines of dangerous
% communities do not reduce offensiveness of the impacted members.} Looking at
% \Cref{fig:moderation:results:banning:offensiveness} and
% \Cref{fig:moderation:results:quarantining:offensiveness},  we can see that
% there is no significant difference in incidence rates of offensive comments
% before and after a ban or quarantine event for our treatment users. Second,
% \emph{impacted community members of bans and quarantines simply move to other
% hate subreddits.} When analyzing the levels of engagement that members of
% banned or quarantined communities had in all hateful communities (including
% those which were soon to be banned), we observed no drop in engagement. In
% fact, we observed that there was an increase in engagement following
% a quarantine -- suggesting that community members continued engagement in the
% quarantined community while also increasing participation in other hateful
% communities.
% 
% We see from \Cref{fig:moderation:results:banning:community}
% that users impacted by community bans continue a high level of engagement in
% other hate communities. Surprisingly, our data shows 
% (\Cref{fig:moderation:results:quarantining:community}) that when communities
% get quarantined, their users typically increase their participation in hate
% communities significantly -- after a lag of several months (and possibly after
% the quarantined community was banned).


%\begin{figure}[th]
  %\centering
  %\begin{minipage}{.485\textwidth}
        %\includegraphics[width=\textwidth]{H3-figs/DBBehaviourChangeAfterBan.png}
        %\caption{Metric: Offensiveness rate. Event: Banning subreddit $\mathfrak{D}_B$.}
        %\label{fig:moderation:results:banning:offensiveness}
    %\end{minipage}
%
%         \label{fig:moderation:results:banning:community}
    %\begin{minipage}{.485\textwidth}
        %\includegraphics[width=\textwidth]{H3-figs/DBBehaviourChangeAfterQuarantine.png}
        %\caption{Metric: Offensiveness rate. Event: Quarantining subreddit in $\mathfrak{D}_B$.}
        %\label{fig:moderation:results:quarantining:offensiveness}
    %\end{minipage}
    %\caption{The impact of ban and quarantine events on user behavior. Month
    %``0'' represents the month of the event. }
    %\vspace{-.25in}
  %\label{fig:moderation:results:intervention}
%\end{figure}
%

\subsubsection{Takeaways: Do ban and quarantine interventions result in
improved user behavior?} \label{sec:moderation:results:takeaways}

Taken together, our analysis shows that participation in problematic
($\mathfrak{D}_I$) subreddits does have an impact on a user's behavior in the
wider community and current administration strategies of bans and quarantines
are not effective for mitigating the impact of this participation on individual
users. Through our results, we are able to \emph{confirm hypothesis H3 -- \ie
problematic behavior is not reduced by bans and quarantines}. This suggests the
need for more nuanced interventions. We note that our validation of H3 actually
contradicts prior work \cite{Chandrasekharan-CSCW2017} which analyzed the bans
of \subreddit{FatPeopleHate} and \subreddit{CoonTown}. We use the same
methodology as they do, however, differences in our findings are for the
following reasons: First, our study is focused on a much larger set of banned
subreddits and is likely more representative of the impact of bans. Second,
there is anecdotal evidence that Reddit's inconsistencies in enforcing
community bans has increased over time.  For example, banning a subreddit $s_1$
has little impact on user behavior when a subreddit $s_2$ exists (and is not
banned) in which the same offensive behavior is encouraged. We note that during
the ban of \subreddit{CoonTown} and \subreddit{FatPeopleHate}, dozens of other
communities with similar ideologies were also banned simultaneously --
effectively deplatforming the ideology. This is not the case with more recent
bans. This refusal to deplatform ideologies results in more potential `homes'
for banned community members to continue their offensive behavior in.  The
quarantine of \subreddit{european} provides an example of this kind of user
migration. Users from \subreddit{european} were seen to migrate heavily to
\subreddit{The\_Donald} \cite{European-Migration}.
%We eventually see 
%\subreddit{The\_Donald} moderators welcoming \subreddit{european} users and
%lifting its no racism rule. 
Finally, previous work has shown that community discourse as a whole has
declined severely in the time since the study of Chandrasekharan \etal and it
is unclear if their research findings still hold in today's climate.

% \subsection{Experiment and Results}\label{sec:moderators:ExperimentRes}
% 
% \textsc{\color{red} This section will describe all the combinations that we tried and will analyze the trends difference between treatment and control users right after inflection points. }
% 
% \subsubsection{Experiment Hypothesis}\label{sec:moderators:ExperimentSetup}
% 
% \textsc{\color{red} This section will tell us what we expect from each experiment iteration. }
% 
% \begin{itemize}
%     \item Offensiveness after joining \textsc{\color{red} Expected Increase in offensiveness}
%     \item Negative participation after joining \textsc{\color{red} Expected Increase in negative participation}
%     \item Offensiveness after subreddit banned \textsc{\color{red} Expected No Effect in offensiveness}
%     \item Negative participation after subreddit banned \textsc{\color{red} Expected No Effect in negative participation}
%     \item Offensiveness after subreddit quarantined \textsc{\color{red} Expected decrease in offensiveness}
%     \item Negative participation after subreddit quarantined \textsc{\color{red} Expected decrease in negative participation}
% \end{itemize}
% 
% \subsubsection{Experiment Results}\label{sec:moderators:ExperimentResults}
% 
% \textsc{\color{red} }
% 
% \begin{itemize}
%     \item Offensiveness after joining
%     \item Negative participation after joining
%     \item Offensiveness after subreddit banned
%     \item Negative participation after subreddit banned
%     \item Offensiveness after subreddit quarantined
%     \item Negative participation after subreddit quarantined
% \end{itemize}
% 
% \subsubsection{Takeaways}\label{sec:moderators:takeaways}


==> old-predictors.tex <==
\section{Identifying Predictors}\label{sec:predictors}

In this section, we use this insight to test the following
hypothesis: \textbf{H2. Evolution into problematic subreddits can be
predicted}. This hypothesis, if valid will show that tools may be built to
help moderators pre-emptively identify and watch subreddits likely to devolve
into problematic subreddits. 
% If invalid, the failed hypothesis will
% show that evolutionary characteristics cannot be used to develop such tools.  
% Our methods and results outlined in \Cref{tab:predictors}.
%  
%  \begin{table}
%    \centering
%    \small
%    \begin{tabular}{ll}
%      \toprule
%      \textbf{Methodological questions} & \textbf{\Cref{sec:predictors:methods}}\\
%      \midrule
%      What evolutionary features do we extract for each subreddit?    & \Cref{sec:predictors:methods:features}\\
%      How do we avoid leakage of features in our classification task? & \Cref{sec:predictors:methods:leakage}\\
%      How do we handle skewed class labels in our classification task?& \Cref{sec:predictors:methods:skew}\\
%      How do we identify the predictive values of features?           & \Cref{sec:predictors:methods:weights}\\
%      \midrule
%      \textbf{Research questions} & \textbf{\Cref{sec:predictors:results}}\\
%      \midrule
%      Can we identify problematic subreddits by their evolutionary features? & \Cref{sec:predictors:results:accuracy}\\
%      What features are predictors of future administrator interventions? & \Cref{sec:predictors:results:features}\\
%      % How far ahead of time can problematic subreddits be identified?        & \Cref{sec:predictors:results:early}\\
%      How well do explainable classifiers do as a real-world administrative tool?   & \Cref{sec:predictors:results:realworld}\\
%      \bottomrule
%    \end{tabular}
%    \caption{Hypothesis 2: Evolution into problematic subreddits can be predicted. Summary of methods and results.}
%    \label{tab:predictors}
%  \end{table}
 

\para{High-level overview.} Our goal is to identify the features that can be
useful to predict the likelihood of a subreddit being classified as problematic
in the future -- \ie can its placement, by Reddit administrators, into
$\mathfrak{D}_I$ be predicted ahead of time. At a high-level, we test this
hypothesis by extracting features from different points in a subreddit's
lifespan and then fitting several explainable classification models assigning
the corresponding labels of $\mathfrak{D}_I$ and $\mathfrak{D}_A$ for each set
of extracted features. We take special care to avoid over-fitting our models
and preventing leakage from impacting our classification task. Our methods
for setting up this classification task are described, in detail, in
\Cref{sec:predictors:methods}. We argue that if our explainable classifiers
have reasonably high F1-score when predicting the future labels assigned to
each subreddit, then the features that are highly weighted by them \emph{must
be good predictors for problematic subreddits, as decided by Reddit
administrators}. We present our results
(\Cref{sec:predictors:results}), which broadly validate our proposed hypothesis
by demonstrating that (1) we can achieve high classification F1-scores with
relatively simple evolutionary features and (2) problematic subreddits can be
identified with reasonable accuracy very early in their lifetime. We also
create a classification task that resembles a real-world setting faced by
administrators and test the usefulness of our classifier. We find that our
explainable classifiers are able to achieve remarkably high performance in
synthetic and natural experimental settings while also shedding light on which
features are inherently most used by administrators in classifying subreddits
as problematic.

\subsection{Methods}\label{sec:predictors:methods}

\subsubsection{What evolutionary features do we extract for each subreddit?}
\label{sec:predictors:methods:features}

For each subreddit in our datasets, we break their lifespan into four quarters
and extract features from each of these quarters. This allows us to do several
things: (1) we are able to get an identical number of features from all
subreddits -- even if they have vastly different lifespan values, and (2) we
are able to capture features from different phases in the evolution of
a subreddit. Our extracted features fall in six categories --
community-, moderator-, user-, structure-, mentions, and language-related
features. These were largely influenced by existing literature seeking to
predict community dynamics (\Cref{sec:related:evolution}). These
features are shown in \Cref{tab:predictors:features} and described below.

\begin{itemize}
  \item \textit{Community-related features.} This category of features captures
    the dynamics of the interactions occurring within the community -- \eg how
    large is the active community, how highly do community members rate each
    others posts, \etc

  \item \textit{Moderator-related features.} Moderators play a large role in
    directing the growth and policies within each community. This category of
    features captures how the moderator team interacts with the community --
    \eg how many moderators does the community has, how many comments are
    deleted by moderators, \etc

  \item \textit{User-related features.} This category of features captures
    characteristics of the average users within the community -- \eg how active
    are users, how frequently do they delete their comments, \etc

  \item \textit{Structure-related features.} We introduce a category of features to
    capture how a subreddit is connected (in terms of shared user base) to other
    communities -- \eg how isolated is the subreddit, what fraction of its
    connections are to other communities which were previously classified as
    problematic, \etc 

  \item \textit{Mention features.} This category of features represent the
    mentions of a subreddit on other subreddits and also in the media. We
    hypothesize that controversial communities are more likely to be referred to
    in on- and off-platform discussions negatively and so these features might
    help distinguish between $\mathfrak{D}_I$ and $\mathfrak{D}_A$. To obtain
    these features, we identified the number of: (1) news articles written about
    the specific subreddit prior to the end of the quarter being studied. The
    dates and article counts were obtained using MIT and Harvard's Media Cloud
    \cite{mediacloud}, an open source platform that gathers and tracks content
    of online news, with the search restricted to their U.S. Top Online News
    collection. (2) references to the specific subreddit on comments made on
    other subreddits. Finally, for both of the types of mentions we compute the
    sentiment towards the community and categorize the mention as either
    negative or not.

  \item \textit{Language features.} This category represents the language
    style of the users in these communities. We use LIWC 2015
    \cite{LIWC} to extract language style features. These features help
    understand the psychometrics of the language within the community In 
    addition to this we use a toxic speech classifier developed by the
    Jigsaw team at Google \cite{perspective} to give probability on
    a comment being precieved as toxic.

  \item \textit{Vocabulary Features.} Finally, this category represents how the
  community is related to other problematic subreddits in terms of shared
  vocabulary. We use vocabulary vectors generated using TF-IDF scores and
  compute the cosine similarity between the community and previously known
  problematic communities.



\end{itemize}

\begin{table}[t]
\small
 	\begin{tabular}{llll}
	\toprule
	{\textbf{Category}}  & {\textbf{Features}}\\ 
	\hline
		& \# active unique commenters		\\
		& \# posts				\\
		& \# comments				\\
		& Dist. of comments \& posts		\\
		& Dist. of score \& comments		\\
		& \% of active user growth		\\
		& Dist. of controversial score per post	\\
		& \# controversial comments		\\
	\multirow{-4}{*}{\textbf{Community}} & \# gilded comments			\\  
	
	\midrule
		& \# moderators				\\
		& \# incomning moderators		\\
		& \# outgoing moderators		\\
		& Dist. of moderators comment score	\\
		& \# AutoModerator comments 		\\
		& Dist. of moderators comment score	\\
		& \# removed posts			\\
	\multirow{-4}{*}{\textbf{Moderators}}
		& \# removed posts score                	\\
	\midrule
	
		& \# active months			\\
	\multirow{-1}{*}{\textbf{Users}}      
		& \# comments by deleted accounts	\\
	\midrule
	
		& \# uniquely connected communities	\\
		& \# total connections			\\
	\multirow{-2}{*}{\textbf{Structural}} 
		& \# users with connections to		\\
		& previously banned communities		\\
	\midrule
		& \# of mentions in other communities 	\\
	\multirow{-1}{*}{\textbf{Mentions}}
		& \# of mentions in popular news outlets	\\
	\midrule
		& 93 standard LIWC 2015 features	\\
	\multirow{-1}{*}{\textbf{Language}}
		& \# Hateful Comments			\\
	\midrule
		& Mean cosine similarity between 	\\
		& vocabulary vectors of previosly	\\
	\multirow{-1}{*}{\textbf{Vocabulary}}
		& banned communities			\\
\bottomrule
\end{tabular}
 \caption{List of features extracted from each quarter of a subreddit's
  lifespan.}
  \vspace{-.25in}
 \label{tab:predictors:features}
\end{table}

% \begin{table}[t]
% \small
%   \begin{tabular}{llll}
%   \toprule
% 	  {\textbf{Category}}  & {\textbf{Features}} & {\textbf{Type}} & {\textbf{Source/}}\\
% 	   &  &  & {\textbf{Methodology}}\\ \hline

% 					  & \# active unique commenters               & Point     & Reddit \\
% 					  & \# posts                                  & Point     & Reddit \\
% 					  & \# comments                               & Point     & Reddit \\
% 					  & Dist. of comments \& posts                & Quartiles & Reddit \\
% 					  & Dist. of score \& comments                & Quartiles & Reddit \\
% 					  & \% of active user growth                  & Point     & Reddit \\
% 					  & Dist. of controversial score per post     & Quartiles & Reddit \\
% 					  & \# controversial comments                 & Point      & Reddit\\ 
%     \multirow{-9}{*}{\textbf{Community}} & \# gilded comments                         & Point      & Reddit\\ 
%     \midrule
% 					  & \# moderators                             & Point     & Reddit \\
% 					  & \# incomning moderators                   & Point     & Reddit \\
% 					  & \# outgoing moderators                    & Point     & Reddit \\
% 					  & Dist. of moderators comment score         & Point     & Reddit \\
% 					  & \# AutoModerator comments 		      & Point     & Reddit \\
% 					  & Dist. of moderators comment score         & Point     & Reddit \\
% 					  & \# removed posts 			      & Point     & Reddit \\
%     \multirow{-7}{*}{\textbf{Moderators}} & \# removed posts score                    & Point     & Reddit \\
%     \midrule
% 					  & \# active months                          & Quartiles & Reddit \\
%     \multirow{-2}{*}{\textbf{Users}}      & \# comments by deleted accounts           & Quartiles & Reddit \\
%     \midrule
% 					  & \# uniquely connected communities         & Point      & Reddit\\
% 					  & \# total connections                      & Point     & Reddit \\
%                                           & \# users with connections to
% 					  previously banned communities      & Point   & Reddit \\
%     \multirow{-2}{*}{\textbf{Structural}} & \% of users with connections to previously banned communities   & Point   & Reddit \\
%     \midrule
% 					  & \# of mentions in other communities       & Point   & Reddit \\
% 	  \multirow{-2}{*}{\textbf{Mentions}} & \# of mentions in popular news outlets      & Point   & Media Cloud \\
%     \midrule
% 	  \multirow{-1}{*}{\textbf{Language}} & 93 standard LIWC 2015 features              & Points   & LIWC\\
% 					& \# Hateful Comments 				    & Points   & HateSonar\\
%     \midrule
% 	  \multirow{-1}{*}{\textbf{Vocabulary}}   & Mean cosine similarity between vocabulary vectors of previosly banned communities  		      & Points  & \Cref{sec:evolution:methods:vectors} \\
%   \bottomrule
% \end{tabular}
%  \caption{List of features extracted from each quarter of a subreddit's
%   lifespan.}
%   \vspace{-.25in}
%  \label{tab:predictors:features}
% \end{table}

\subsubsection{How do we avoid leakage of features in our classification task?}
\label{sec:predictors:methods:leakage}

Extracting features without careful considerations can result in leakage that
impacts the quality of the classification task. To avoid this problem we need
to make sure that features used in our task are actually available for use, by
administrators, at the time of the classification task. For example in Q1 of
a subreddit's lifetime which may be between months $m_1$ and $m_2$, we cannot
extract features which might rely on data from after $m_2$. This is
particularly important when considering the features in the structural and
mentions categories. In our feature extraction process for each subreddit, we
take care to only consider information available from each quarter. For
example, when extracting the `\% of users with connections to previously banned
communities' structural feature we only consider connections with communities
which were banned \emph{before the end of the corresponding quarter for the
corresponding subreddit}. Furthermore when creating topic vectors, the
vocabulary is limited to tokens observed only during the timespan 
of our training.
Therefore, our feature sets are all obtained from data that is available to
administrators at the time of classification and is amenable to leakage-free
classification. The classification performance results shown in
\Cref{sec:predictors:results} are therefore representative of the effectiveness
of the classifier given the information available to administrators \emph{at
the end of each quarter of each subreddit's lifespan}.

\subsubsection{How do we handle imbalanced class labels in classifier model
training?} \label{sec:predictors:methods:skew}

Our dataset has a severe imbalance of class labels with only 246
$\mathfrak{D}_I$ subreddits and 3K $\mathfrak{D}_A$ subreddits. We take care to
address the model-building and performance-reporting challenges that arise from
this imbalance.

\para{Addressing imbalanced classes in model training.} We used and evaluated
multiple techniques to handle imbalance classes while training -- oversampling
from the minority class ($\mathfrak{D}_I$) using using  Adaptive Synthetic Sampling (ADASYN) \cite{adasyn} and
undersampling from the majority class ($\mathfrak{D}_A$) using ensemble learning
\cite{Zhu-CDL2013}

\begin{itemize}
\item \textit{Approach 1: Oversampling $\mathfrak{D}_I$.} ADASYN
  oversampling works by creating synthetic samples from the minority
  class. ADASYN is very similar to other synthetic oversampling techinques
  such as the SMOTE algorithm /cite{Chawla-IJCAI2002}. However, unlike
  SMOTE, ADASYN adaptively creates synthetic points while considering the
  neighborhoods of the class borders. Consequently, this, compared to
  other oversampling methods, generates synthetic points near the class
  borders as well and therefore mitigating the overfitting problem SMOTE
  has. For the purposes of training our model, we used ADASYN to create
  a perfectly balanced dataset with equal $\mathfrak{D}_I$ and
  $\mathfrak{D}_A$ datasets. Validation and testing were carried out only
  on samples not used or generated by ADASYN.
  
\item \textit{Approach 2: Undersampling $\mathfrak{D}_A$.} Our
undersampling approach works by: (1) splitting the training samples of the
majority class ($\mathfrak{D}_A$) into equal sized datasets
($\mathfrak{D}_{A_1}$, $\mathfrak{D}_{A_2}$, \dots, $\mathfrak{D}_{A_n}$)
with the number of samples in each dataset equal to the total number of
minority class ($\mathfrak{D}_I$) training samples, (2) training a set of
classifiers, $c_1$ \dots $c_n$, with each using one of newly split
majority class datasets and the entire minority class training samples as
training input -- \ie classifier $c_i$ trains on samples from
$\mathfrak{D}_{A_i}$ and $\mathfrak{D}_I$, and (3) assigning the label
output by the majority of the $n$ classifiers when given a feature set for
classification into $\mathfrak{D}_I$ or $\mathfrak{D}_A$.
\end{itemize}

Results for both sampling approaches are comparable and reported in
\Cref{sec:predictors:results}. We note that these approaches were utilized
\emph{only for expanding the training sets used and did not impact the testing
and holdout datasets} in our classification experiments.

\para{Addressing imbalanced classes in reporting of classifier performance.} The
imbalance (1:12) of class labels in our dataset means that it is possible for
model to report over 92\% accuracy by simply guessing that every feature set
came from a $\mathfrak{D}_A$ subreddit. We avoid such pitfalls by reporting the
area under the ROC curve widely used for evaluating classifiers trained on
imbalanced datasets. We also report the individual F1-scores for each of the
classes.

\subsubsection{How do we identify the predictive value of features?}
\label{sec:predictors:methods:weights}

Given labels for each subreddit and a set of features associated with each
stage in its lifetime, we now seek to understand the predictive values of these
features. We achieve this in two steps: First, we build a machine learning
classifier model which uses these features to predict the labels associated with
each subreddit. Next, for high-performing classifiers, we analyze the weights
associated with each feature by the classifier. Our argument is that \emph{if
a classifier is able to achieve a reasonably high F1-score, then the features
it weighs heavily must have some predictive value}. We focus solely on
interpretable classifier models (logistic regressions, decision trees, and
random forests) since we need to obtain feature weights. However, we see very
similar classifier performance, when comparing our models to other
non-interpretable models such as SVMs. Below we explain how we train, validate,
test, and interpret our models.

\para{Classifier model training, validation, and testing.} To evaluate the
performance of each classifier model we first split the samples in our dataset
with 80\% of each class randomly allocated for training and validation and the
remaining 20\% reserved for holdout testing. We then used five-fold
cross-validation to evaluate the classifier performance on the training and
validation dataset -- expanding \emph{only the training samples} with the
sampling approaches detailed in \Cref{sec:predictors:methods:skew} in each
fold. Finally, we evaluated the classifier performance on the holdout set. In
our results we report the mean F1-score in the 5-fold cross-validation as well
as on the holdout test samples.

\para{Interpreting logistic regression models.} {Logistic Regression} models
a relationship between an outcome variable $y$ and a group of predictor
variables in terms of log odds. In order to interpret the model, we compute the
estimated weights for each feature and their corresponding odds ratio
\cite{ML-Interpret}. If the odds ratio for a feature ($f$) is $x$, it means
that a unit increase in $f$ changes the odds of our outcome variable $y$ by
a factor of $x$ when all other features remain the same. By calculating the
features with the highest odds ratios for different labels, we are able to
identify which features are the best predictors of problematic subreddits, as
later decided by Reddit administrators.

\para{Interpreting decision tree and random forest models.} Tree based models
are the easiest to interpret. We find the importance of each feature using Gini
Importance \cite{Breiman-Gini}. At a high-level the Gini importance counts the
number of times a feature is used as a splitting variable, in proportion with
the fraction of samples it splits. For random forests, the Gini importance is
averaged over all the constructed trees. We expect more important features to
have higher Gini importance scores. Unlike logistic regression interpretation,
a limitation here is that this metric only allows us to rank feature
importance, but not quantify the relative difference of their importance.

\subsection{Results}\label{sec:predictors:results}

%We now focus on measuring the effectiveness of using evolutionary features to
%predict which category (from dangerous/banned, hateful, and benign) subreddits
%belong to (\Cref{sec:predictors:results:accuracy}), which features are the best
%predictors of subreddit behavior (\Cref{sec:predictors:results:features}), and
%the impact of observation time on classifier accuracy
%(\Cref{sec:predictors:results:early}). Our results are summarized in 
%\Cref{tab:predictors:results}.

\subsubsection{Can we identify problematic subreddits by their evolutionary
features?} \label{sec:predictors:results:accuracy}

\begin{table*}[t]
  \small
  \begin{subtable}[t]{\textwidth}
  \centering
	\begin{tabular}{l l l l l}
    \toprule
    \textbf{Model} & \multicolumn{4}{c}{\textbf{Classifier Performance
%    (\%AUC, \%F1-Negative, \%F1-Positive, \%F1)}}  \\\cmidrule{2-5}
%	   &  Q1 & Q1+Q2 & Q1+Q2+Q3 & Total \\\midrule
%	  Random Forest  & (93, 97, 68, 94) & (95, 98, 78, 96) & (96, 99, 84, 98) & (97, 99, 88, 98) \\
%	  Logistic regression  & (79, 79, 59, 78) & (80, 81, 60, 79) & (79, 83, 65, 76) & (85, 92, 70, 83) \\
    (\%AUC, \%F1-Negative, \%F1-Positive)}}  \\\cmidrule{2-5}
	   &  Q1 & Q1+Q2 & Q1+Q2+Q3 & Total \\\midrule
	  Random Forest  & (93, 97, 68) & (95, 98, 78) & (96, 99, 84) & (97, 99, 88) \\
	  Logistic regression  & (79, 79, 59) & (80, 81, 60) & (79, 83, 65) & (85, 92, 70) \\
    \bottomrule
  \end{tabular}
  \caption{Performance of classifiers built using ADASYN oversampling during
    training.}
  \label{tab:predictors:results:accuracy:oversample}
  \end{subtable}
  \caption{Performance of our classifiers in predicting $\mathfrak{D}_I$ and
  $\mathfrak{D}_A$ labels at the end of each quarter of a subreddit's lifespan
  while using ADASYN oversampling in model training.
  Q1 denotes that the classifier only had access to features from the first
  quarter of each subreddit's lifespan, Q1+Q2 denotes access to features from
  the first two quarters, Q1+Q2+Q3 denotes access to features from the first
  three quarters, and Total denotes access to features from the entire
  lifespan. Values denote area under the ROC, F1-score for negative subreddits,
  F1-scores for positive subreddits on the holdout set.}
  \label{tab:predictors:results:accuracy} \end{table*}

Column ``Total'' of \Cref{tab:predictors:results:accuracy} shows how our
different explainable classifier models performed at classifying subreddits
into $\mathfrak{D}_I$ and $\mathfrak{D}_A$ when given access to all
evolutionary features of the subreddit, as would be available at the end of the
quarter Q4 of a subreddit's lifespan (which for $\mathfrak{D}_A$
subreddits is the last month of data used in this study -- 04/2020). As we
can see all our models perform remarkably well, achieving AUC-ROC as high
as 97\% on our holdout set, regardless of whether models were built using
ADASYN oversampling or majority class undersampling. More interestingly,
we notice that our Random Forest classifiers are able to achieve high
AUC-ROC even as early as after Q1 (93\%) with
performance only increasing with longer observations of a subreddit's
evolution. These results indicate that, by observing the evolutionary
features described in \Cref{sec:predictors:methods:features}, problematic
subreddits can be identified much earlier than they currently are.
Further, the performance of our interpretable classifiers are reasonable
enough to warrant their use to understand feature importance and the
predictors of problematic subreddits.

% \subsubsection{How reactive is Reddit moderation to the media?}
% \label{sec:predictors:results:media}
% In \Cref{sec:introduction} we claimed that Reddit
% administrative actions were heavily driven by media criticism and therefore
% reactionary rather than proactive. To validate this claim, we removed all
% `mention'-related features from our classifier and compute its F1-score. We
% find that F1-score for the banned class drops to 76\%. While inspecting the
% confusion matrices obtained from our testing, we see that our classifiers had
% problems in distinguishing between subreddits with `banned' and `hate' labels
% (the F1-score for benign subreddits was 81\%). Including mentions-related
% features mitigates this problem. This result implies that: (1) while
% media-mentions are not predictive of hateful subreddits, they are predictive of
% banned subreddits (\ie these are predictive of admin reactions) (2) our
% classifier continues to have reasonable performance even when accounting for
% the absence of media-mention features, and (3) our classifier performs very
% well at filtering out benign subreddits -- thus showing its usefulness as a
% filtering tool for moderators.

\subsubsection{What features are most important for predicting the evolution
into problematic subreddits?} \label{sec:predictors:results:features}

\begin{table}[t]
\small
  \begin{tabular}{lp{0.6in}p{0.6in}}
  \toprule
    {\textbf{Feature}}  & {\textbf{RF feature rank}} & {\textbf{LR log odds ratio}} \\
%   {} & {\textbf{Feature rank}} & {\textbf{log odds ratio}} \\
    \hline
    \# users connected to \\
    previously banned communities & 1   &   0.32\\
    \# average percentage \\
     of toxic comments score & 2 & 0.20 \\
    \# negative mentions \\
     in other communities& 3 & 0.24 \\
    \# percentage of \\
    comments removed & 4 & 0.18\\
    \# negative mentions\\
     in media outlets & 5 & 0.20\\
  \bottomrule 
  \end{tabular}
  \caption{List of top-5 most predictive features for our random forest
  (RF) and logistic regression (LR) classifiers. The top-4 features were
  identical in both models, although with slightly different ordering of
  importance.}
  \label{tab:predictors:results:features} 
\end{table}

\Cref{tab:predictors:results:features} shows the top-5 most important
features as determined by our random forest and logistic regression
classifier models. Here, we see that the most predictive feature in both
models is the number of users who were previously active on communities
that were previously banned. This feature has a log-odds ratio of .32
indicating that a unit increase in the number of users connected to
previously banned communities resulted in a 1.37x increase in the odds of
the subject subreddit being categorized as problematic. Similarly, we see
increases ranging from 1.19x to 1.27x in the odds of the subject subreddit
being categorized as problematic per unit increase in the average
percentage of toxic comments, number of negative mentions in media and
other communities and percentage of comments by removed.
These results suggest that: (1) communities which entertain users with
interactions in previously banned communities have a significantly higher
likelihood of becoming problematic as well -- suggesting that
administrator interventions on problematic subreddits, rather than users
of problematic subreddits is not entirely effective at preventing the
re-occurrence of problematic subreddits, and (2) Reddit administrators are
indeed more likely to intervene when a community gets negative attention
in media or other communities -- although we cannot make a causal claim
here, the evidence suggests a strong positive correlation.

% \subsubsection{How far ahead of time can hateful or dangerous subreddits be
% predicted?} \label{sec:predictors:results:early}
% Our goal goes beyond identifying the labels associated with a subreddit. Since
% we are motivated by the need for tools to aid proactive (and early) community
% interventions, we also need to understand how early the future behavior of
% a subreddit can be predicted. To this end, we evaluated each classifier's
% performance using features extracted only from the first quarter (Q1), first
% half (Q1+Q2), and first three-quarters (Q1+Q2+Q3) of a subreddit's lifespan.
% %For reference, subreddits in $\mathfrak{D}_B$, which we label as dangerous, had
% %the following lifespan distribution [$\min$: 7 months, $25^{th}$ percentile: 20
% %months, median: 34 months, $75^{th}$ percentile: 39 months, $\max$: 43
% %months]\footnote{These are lower bounds on lifespan of dangerous/banned
% %subreddits since our data collection only started in 01/2015 and subreddits in
% %$\mathfrak{D}_B$ might have been active before our data collection began.}. 
% From the results shown in \Cref{tab:predictors:results}, we see that while
% features from Q4 are the most important for all our models, the random
% forest and logistic regression classifier has consistently strong
% predictive performance even from first quarter of the subreddit's lifespan.
% \emph{This shows that even features chosen from early in the subreddits
% lifetime (\eg Q1) can be predictors of future subreddit behavior}. This finding
% strongly reinforces the feasibility of early and pre-emptive interventions to
% correct subreddit behavior. We note that our classifiers were able to predict
% the quarantining of \subreddit{The\_Donald} before the actual intervention in
% 06/2019.
% 
% In particular, several hate subreddits (\eg \subreddit{The\_Donald} and
% \subreddit{inceltears}) were consistently misclassified as dangerous/banned
% subreddits due to very similar evolutionary patterns. We note that since our
% classes rely on human coding (\ie our banned/dangerous subreddits are
% essentially labeled by Reddit administrators), it is not clear if these
% misclassifications are a result of inadequate features or inconsistent
% application of content policies by Reddit administrators (although a cursory
% qualitative analysis of the content in \subreddit{The\_Donald} suggests the
% latter). 
% 

\subsubsection{How well do explainable classifiers do as a real-world
administrative tool?}\label{sec:predictors:results:realworld}

Our previous results, reported in \Cref{sec:predictors:results:accuracy},
reflect our classifier performance over the entire dataset of $\mathfrak{D}_I$
and $\mathfrak{D}_A$. We now seek to understand how well our classifier would
perform in a real-world deployment as a tool to aid Reddit administration. To
this end, we trained our classifier on features obtained from $\mathfrak{D}_I$
and $\mathfrak{D}_A$ prior to 03/2018 and evaluated our classifier performance
and agreement with Reddit's administrative intervention decisions made from
03/2018 onwards. During this time, Reddit performed ad ministrative ban
and quarantine interventions on 130 subreddits – of these our classifier
agreed with 86 intervention decisions and achieved an AUC-ROC of 84. Out
of these 130 subreddits, 52 subreddits experienced administrative
intervention because of reasons related to toxicity, while the rest were
intervened because of violations on rules ranging from piracy, spam and
porn.

Examples of the subreddits that our classifier identified as problematic correctly:

\begin{itemize}

\item r/Braincels was the most popular subreddit for incels, or
"involuntary celibates", after r/Incels was banned, gaining 16,900
followers by April 2018. The subreddit's leaders decided to ban
individuals advocating for murder.[9] However, the subreddit promoted rape
and suicide.[10] The subreddit was banned in September 2019, after
violating Reddit's Content Policy with respect to bullying and
harassment.[11][12][13]

\item Mr\_Trump Banned In November 2019, the subreddit's moderators
attempted to evade Reddit's imposed quarantine by reviving and promoting
a subreddit called r/Mr\_Trump. This subreddit was banned by Reddit's
administrators in accordance with its policy that "attempting to evade
bans or other restrictions imposed on communities is not allowed on
Reddit".[70] Days later, Reddit's admins warned the subreddit's moderators
about trying to out the alleged White House whistleblower in the
Trump–Ukraine scandal in violation of Reddit's rules on harassment and
inviting vigilantism.

\item FrenWorld Banned June 2019  "/frenworld along with several other
similarly themed subreddits, was, on its face, largely dedicated to
posting "frenly" (friendly) content about frogs in clown wigs and speaking
in a sort of pseudo-baby-talk. Underneath this face was a subtext of
racism and violence. They would refer to Jewish people as "nose-frens",
for example. Anyone who disagreed or disliked the sub was a "non-fren".
They would advocate violence by saying that people needed to get "bopped"
which was really just another way to say "killed". There was a lot of Nazi
imagery, and the comments referenced other racist memes, such as "13%", "6
million", and things like that."

\item The\_Europe r/the\_europe was known for stuff like holocaust denial
and all sorts of racism, and got banned for that.

\item Ice\_Posieden2 Secondary subreddit after Ice\_Posieden which was
also banned

\item A lot of piarcy subreddits such as sports\_hd\_online,
PackersVikingsLiveHd, soccerstreams, fullmoviesonanything

\item A lot of pornographic subreddits such as InstaThots,
WilderFuryLiveHd, CelebJOMaterial

\item others casualChildAbuse

\end{itemize}

Examples of subreddits identified as problematic but were not classified as
such by administrators.

\begin{itemize} 
\item AskTrumpSupporters 
\item france. A lot of anti muslim top rated posts regarding the blasphemy
incident 
\item engrish Slightly racist posts? 
\item Enoughsandersspam 
\item A lot of porn 
\item A lot of gaming subs 
\item Some private subs 
\item FreeKarma4You 
\item VitaPiracy
\end{itemize}


Examples of the 18 subreddits that our classifier identified as problematic but
were not classified as such, by administrators, were \subreddit{RedPillWomen}
and \subreddit{marriedredpill} -- subreddits associated with previously banned
subreddit \subreddit{TheRedPill}. Examples of the 7 subreddits that our
classifier failed to identify the quarantining of \subreddit{EdgyMemes} and
\subreddit{Ice\_Poseidon}  -- subreddits which were banned for bullying and
harassment. These results suggest that our classifier is usable as a real-world
administrative aid to help administrators identify and monitor potentially
problematic subreddits. We plan to release, along with our models, monthly
updates of the subreddits identified as problematic by our models (along with
their feature sets) at \url{https://anonymized.for.review} after peer review of
this manuscript.

\subsubsection{Takeaway: Can evolution into problematic subreddits be
predicted?} \label{sec:predictors:results:takeaway}
Our results show that evolutionary features can not only be


used to identify subreddits likely to be identified as problematic, by Reddit
administrators, in the future. We showed that the most informative feature
used by our classifier is the fraction of users with prior activity in
other subreddits that had previously violated platform guidelines. This
finding suggests that administrative interventions might be more
beneficial when they are focused on problematic users, rather than
problematic subreddits. Further, we also showed that media reporting of
discourse on Reddit is a strong predictor of Reddit's action on known
hateful communities. Taken all together, we are able to confirm that
\emph{evolution into problematic subreddits can be predicted -- \ie
hypothesis H2 is valid}. This suggests that administrator and community
moderation tools, that are able to identify potentially problematic
subreddits requiring careful monitoring, are possible.


==> old_evolution.tex <==
\section{Subreddit Evolution and Convergence}\label{sec:evolution}

In this section, we focus on testing the following hypothesis:  \textbf{H1.
Subreddits may not converge to topical and user base stability}. If valid, this
hypothesis demonstrates the need: (1) for computational techniques to monitor
subreddit evolution (in terms of topics and user bases) and (2) to frequently
evaluate the suitability of making administrative interventions. Additionally,
such analysis may yield insights into the potential for identifying
evolutionary patterns that can serve as early predictors for subreddits likely
to require future administrator interventions. If invalid, the failed
hypothesis will show that subreddits converge to topical or user base stability
and therefore only need to be evaluated by administrators once -- after
stability has been reached. This will invalidate the need for computational
tools since the constant monitoring of subreddits is unnecessary. Our methods
and results are outlined in \Cref{tab:evolution}.

\para{High-level overview.} Our goal is to identify if subreddits reach
topical or user stability -- \ie if the topics of discussion and users
participating in these discussions stabilize over time. In order to accomplish
this goal, we need a technique to quantify the (dis)similarity in topics and
user bases for a subreddit at two points in time. 
%
We accomplish this using the following approach, which is explained in more
detail in \Cref{sec:evolution:methods}. First, for each month of activity in
each subreddit (which we refer to as a \emph{subreddit state}), we generate
a pair of fixed-length vectors --  a vector representative of the topics being
discussed in posts and comments in the subreddit (\ie a topic vector) and
a vector representative of active users in the subreddit (\ie an active user
vector) using TF-IDF and active user co-occurrence matrices, respectively.
Next, we leverage two measures to quantify changes (or evolutionary distance)
between these vectors -- an absolute measure (\ie cosine similarity between two
given vectors) and a relative measure (\ie the Kendell tau distance between the
ordered list of nearest neighbors of the two given vectors). Both of these are
described in more detail in \Cref{sec:evolution:methods}. Using both methods,
we find that subreddits generally do not converge to a stable set of topics or
active users -- \ie they continue to evolve throughout their lifespan. This
validates our proposed hypothesis. Detailed results are presented in
\Cref{sec:evolution:results}.

\begin{table}
  \centering
  \small
  \begin{tabular}{ll}
    \toprule
    \textbf{Methodological questions} & \textbf{\Cref{sec:evolution:methods}}\\
    \midrule
    How do we convert \emph{subreddit states} into fixed-length vectors
    representing topics and active users? & \Cref{sec:evolution:methods:vectors} 
    \\
    How do we compute the \emph{absolute distance} between two topical or user
    base subreddit states? & \Cref{sec:evolution:methods:cosine}
    \\
    How do we compute the \emph{relative distance} between two topical or user
    base subreddit states? & \Cref{sec:evolution:methods:clustering}
    \\
    \midrule 
    \textbf{Research questions} & \textbf{\Cref{sec:evolution:results}}\\
    \midrule
    Do subreddits converge to topical stability? & \Cref{sec:evolution:results:topics} 
    \\
    Do subreddits converge to user base stability? & \Cref{sec:evolution:results:users}
    \\
    Do subreddits in $\mathfrak{D}_I$ have different evolutionary behaviors
    than subreddits in $\mathfrak{D}_A$? & \Cref{sec:evolution:results:differences}
    \\
    \bottomrule
  \end{tabular}
  \caption{Hypothesis 1: Subreddits may not converge to topical or user
  stability. Summary of methods and results.}
  \label{tab:evolution}
\end{table}

 
% Second, we perform hierarchical clustering on both types of vectors across all
% the subreddit states in our dataset. We then quantify the \emph{evolutionary
% distance} of topics or active users between any two states of a specific
% subreddit as the \emph{height of the nearest common parent} in our topic or
% active user hierarchical clusters, respectively. 
% % We claim that the topics or user base of a subreddit ($s$) has \emph{converged}
% % between times $t_1$ and $t_2$ if the evolutionary distance between the
% % corresponding vectors at these timestamps is minimum. 
% We present our results, which broadly (\ie for all categories of subreddits in
% our study) validate the proposed hypothesis in \Cref{sec:evolution:results}.
% 
\subsection{Methods}\label{sec:evolution:methods}

% Our method for testing the hypothesis involves two steps: First, we create
% latent vector summaries of topics and user participation for each subreddit
% state (\Cref{sec:evolution:methods:lsa}). Next, we measure the similarities of
% these summaries as a function of time (\Cref{sec:evolution:methods:clustering}).
% 
\subsubsection{How do we convert subreddit states into fixed-length vectors
representing topics and active users?}\label{sec:evolution:methods:vectors}

Recall, a \emph{subreddit state} is all the activity associated with
a subreddit during a given month -- \eg the subreddit state associated with
\subreddit{politics} on 09/2019 contains all user posts and comments made on
\subreddit{politics} during the month of 09/2019. Our goal is to create two
fixed-length vectors which capture: (1) the topics associated with each
subreddit state and (2) the active user base associated with each
subreddit state.

\para{Creating fixed-length topic vectors for each subreddit state.} At
a high-level, our topic vector for each subreddit state is the vector of Term
Frequency - Inverse Document Frequency (TF-IDF) \cite{Sparck-DRS1988} weights
associated with each unique token in our dataset. This is a standard document
representation approach in the information retrieval community
\cite{Beel-IJDL2016} to associate keywords with documents. We apply this
approach as follows:
\begin{itemize}
  \item \textit{Random sampling and document corpus creation.} We begin by
    randomly sampling 10\% of all comments in our dataset (a necessity owing to
    the large dataset and computational limitations). The sampled comments are
    then used to create documents associated with each subreddit state -- \eg
    the document associated with the (\subreddit{news}, 09/2019) subreddit
    state will contain all the sampled comments which were made by users on
    \subreddit{news} during the month of 09/2019. At the end of this step, we
    have a corpus of documents ($D$) containing one document for each
    subreddit state in our dataset. \rnnote{If we have time, we should repeat
    this for 5-10 independent samples and show statistical significance of our
    analysis across all samples.}
  \item \textit{Text pre-processing and token corpus creation.} We perform
    standard text pre-processing operations including removing English stop
    words, tokenization, and lemmatization for each document. The unique
    tokens, across $D$, at the end of this pre-processing stage form the corpus
    of words and determine the length of the vectors associated with each
    subreddit state. At the end of this step, we have a corpus of all unique
    lemmatized tokens ($T$) observed in $D$. The length of the topic vector
    associated with each subreddit state is $|T|$.
  \item \textit{Computing topic vectors for each subreddit state.} For each
    document $d \in D$, we compute the TF-IDF weight of each token $t \in T$.
    Therefore the $i^{th}$ entry in the topic vector for $d$ is
    ${f(t_i)}\times{\log\frac{|D|}{|D_{t_i}|}}$, where $f(t_i)$
    denotes the frequency of token $t_i$ in $d$ and $D_{t_i}$ is the set of all
    documents containing the token $t_i$. A high TF-IDF weight for a (document,
    token) pair indicates that the token has a high frequency of occurrence in
    the given subreddit state document and a low frequency of occurrence in all
    other subreddit state documents -- \ie the token is of high importance in
    the given subreddit state document. Therefore, the topics associated with
    each subreddit state are represented by a vector denoting the importance of
    each token (observed in $D$) with respect to all sampled comments made on
    the subreddit during the corresponding month.
\end{itemize}


\para{Creating fixed-length active user vectors for each subreddit state.} At
a high-level, our active user vector for each subreddit state is the vector of
fraction of active user co-occurrences with other subreddit states. This is
a standard technique used in collaborative filtering and recommender systems
research \cite{Liang-RecSys2016, Dunning-2014} to identify shared interests
between sets of users or communities. We apply this approach as follows:
\begin{itemize}
  \item \textit{Active user identification.} We begin by creating sets of
    active users for each subreddit state in our dataset. Active users
    associated with a subreddit state are identified as all users with any
    posting or commenting activity on the corresponding subreddit during the
    corresponding month. We refer to the set of active users of subreddit state
    $s$ as $A_s$. We note that active user vectors are created using the
    complete dataset without sampling.
  \item \textit{Computing active user vectors for each subreddit state.} For
    each subreddit state, we compute the fraction of active users who overlap
    with every other subreddit state. The $j^{th}$ entry in the active user
    vector for subreddit state $i$ corresponds to the fractional overlap with
    subreddit state $j$ -- \ie it has the value $\frac{|A_i \cap
    A_j|}{|A_i|}$. A higher overlap ratio indicates that the two subreddit
    states share a larger cohort of users. Therefore, the active users of
    a subreddit state are represented by a vector denoting the sizes of the
    cohorts shared with all other subreddit states. The length of this vector
    is equal to the total number of subreddit states in our dataset.
\end{itemize}

\subsubsection{How do we compute the absolute distance between two
subreddit states?} \label{sec:evolution:methods:cosine}
Our goal is to measure the absolute distance between two subreddit states. In
other words, the measure needs to be completely independent of the effect of
changes occurring on other subreddit states.

\para{Absolute distance measures and their relationship with subreddit
evolution.} Absolute distance measures, in the context of subreddit states,
allow us to quantify how topics or user bases have evolved without accounting
for changes in discourse or participation dynamics on other parts of the
platform. For example, consider the states associated with (\subreddit{news},
11/2019) and (\subreddit{news}, 04/2020). The absolute distance between the
topic vectors associated with these subreddits will be large  owing to the
significant change in discourse topics (\ie from American primary elections to
COVID-19) regardless of the fact  that many other news-related subreddits (\eg
\subreddit{usnews} or \subreddit{worldnews}) were also heavily focused on
American politics in 11/2019 and COVID-19 in 04/2020. Analysis with an absolute
measure therefore automatically includes the effect of global or platform-wide
changes to topic or active user base evolution for a subreddit. We say that
subreddits have converged if the absolute distance computed over topic and
user vectors from consecutive months converges at the minimum -- \ie
a similarity score of 1 for the measure described below.

\para{Quantifying absolute distance using cosine similarity scores.}
Given two vectors of identical length ($A$ and $B$) which represent either
topic or active user base vectors of two subreddit states, the absolute
distance measure uses the cosine similarity score between them (\ie $similarity =
\frac{\sum_{i=1}^{n}{A_iB_i}}{\sqrt{\sum_{i=1}^{n}A_i^2}\sqrt{\sum_{i=1}^{n}B_i^2}}$).
This measure computes the angular distance between the two vectors without any
consideration of the vectors generated by any of the other subreddit states on
the platform. A high cosine similarity score ($\approx 1$) is indicative of
a very small absolute distance between the two vectors and conversely a low
cosine similarity score ($\approx 0$) is indicative of a large absolute
distance between the two vectors. In the context of topic vectors, a high
similarity score (which corresponds to a low absolute distance) indicates that
there are many keywords which share high importance (as computed by TF-IDF
weights) on both subreddit states. In the context of active user vectors,
a high similarity score (which corresponds to a low absolute distance)
indicates that the active users of the two subreddit states also share similar
levels of participation (as computed by active user co-occurrence fractions) in
many other subreddit states.

% \begin{figure}[t]
%    \centering
%         \includegraphics[width=.49\textwidth]{H1-cat-figs/topic-cluster-evolution.pdf}
%         \includegraphics[width=.49\textwidth]{H1-cat-figs/topic-cluster-monthly.pdf}\\
%         \includegraphics[width=.49\textwidth]{H1-cat-figs/topic-similarity-evolution.pdf}
%         \includegraphics[width=.49\textwidth]{H1-cat-figs/topic-similarity-monthly.pdf}
% 	\hhnote{topic-evolution-cluster, topic-monthly-cluster, topic-evolution-similarity, topic-monthly-similarity}
%   \label{fig:moderation:results:joining}
% \end{figure}

\subsubsection{How do we compute the relative distance between two
subreddit states?} \label{sec:evolution:methods:clustering}
Here, in contrast with absolute distance measures, our goal is to define the
distance between two subreddit states as a function of all other subreddit
states in our dataset. In other words, our measure needs to track subreddit
evolution while accounting for the effects of changes occurring on other
subreddit states.

\para{Relative distance measures and their relationship with subreddit
evolution.} Relative distance measures, in the context of subreddit states,
allow us to quantify how a subreddit's topics and user bases have evolved as
a function of the topics and user bases of other subreddits. For example, let
us once again consider the states associated with (\subreddit{news}, 11/2019)
and (\subreddit{news}, 04/2020). The relative distance between the topic
vectors associated with these subreddits will account for the fact that
although the absolute change between the vectors is large due to the change in
discussion topics from American primary elections to COVID-19, the changes with
relative to other subreddits is smaller -- \ie subreddits (\eg
\subreddit{usnews}) which shared similar topics with \subreddit{news} in
11/2019 still shared similar topics in 04/2020. Analysis with a relative
distance measure therefore identifies how much subreddits have changed with
respect to their neighbors and how their role on the platform has changed. We
say that subreddits have converged if the relative distance computed over topic
and user vectors from consecutive months converges to the minimum -- \ie
a correlation score of 1 for the measure detailed below.

\para{Quantifying relative distance using the Kendall rank correlation scores.}
Given two vectors of identical length which represent either topic or active
user base vectors of two subreddit states, we perform the following operations
to obtain their relative distance.
\begin{itemize}
  \item \textit{Generate list of neighbors ordered by euclidean distances.} Let
    $v_1$ and $v_2$ be the two input (topic or user base) vectors, associated
    with subreddit states $s_1$ and $s_2$ and belonging to months $m_1$ and
    $m_2$, whose relative distance we wish to compute. Let $S_{m_1}$ be the set
    of all subreddit states from month $m_1$ and $S_{m_2}$ be the list of all
    subreddit states from $m_2$. We begin by computing the euclidean distances
    between (1) $v_1$ and every subreddit state in $S_{m_1}$ and (2) $v_2$ and
    every subreddit state in $S_{m_2}$. Finally, we sort the elements of
    $S_{m_1}$ and $S_{m_2}$ in ascending order of their euclidean distance to
    $v_1$ and $v_2$ and store these ordered lists in $X_1$ and $X_2$,
    respectively. These lists are effectively the neighbors of $s_1$ and $s_2$
    ordered from nearest to farthest.   
  \item \textit{Computing the Kendall rank correlation scores.} Given the
    ordered lists of neighbors, $X_1$ and $X_2$, we then compute the Kendall
    rank correlation score between them. This measure computes the level of
    agreement between the two ordered lists. A high Kendall rank correlation
    score ($\approx 1$) indicates that the two lists have nearly identical
    ordering and is indicative of a very small relative distance between
    the subreddit states $s_1$ and $s_2$ -- \ie they are located in the same
    \emph{neighborhood} on Reddit. Conversely, a low rank correlation
    score ($\approx -1$) indicates that the two lists have larger relative distance
    between them -- \ie they are located in distant neighborhoods on Reddit.    
\end{itemize}

% Given succinct vector representations of subreddit states, we now need to
% quantify the distance between these representations. We do this by using
% \emph{agglomerative cluster distance} as a measure of distance between
% subreddit states.
% % 
% % A simple approach is to
% % rely on euclidean distances between the vectors of two subreddit states.
% % However, this would require thresholds and would fail to provide the
% % \emph{nature} (direction relative to other communities) of evolution. We
% % overcame these limitations by relying on \emph{agglomerative cluster distance}
% % as a measure of distance between subreddit states.
% % 
% %however, there are two main drawbacks with this approach: (1) it is not clear
% %what a euclidean distance threshold must be for us to claim that subreddit
% %states have converged and (2) the euclidean distance metric is not suitable
% %for measuring the \emph{nature} of subreddit evolution -- \ie the direction
% %(relative to other communities) of evolution in terms of topics and active user
% %bases. We overcome these limitations by relying on \emph{agglomerative cluster
% %distance} as a measure of distance between subreddit states. 
% 
% % \begin{figure}[t]
% % \includegraphics[width=\linewidth]{evolution-figs/Dendrogram2.pdf}
% % \caption{An snippet of a larger dendrogram obtained by hierarchical clustering
% %   on topic vectors. LDA topics are associated with each cluster.}
% % \label{fig:evolution:methods:dendro}
% % \end{figure}
% % 
% 
% \para{Creating subreddit state clusters.} We performed clustering separately on
% 	user and topic vectors. In both cases, we used agglomerative (bottom-up)
% 	hierarchical ward-method clustering \cite{murtagh2014ward}. In agglomerative
% 	clustering, typically visualized as a dendrogram, clusters at higher levels are
% 	larger and more general while clusters at lower levels are much smaller and
% 	specific. Agglomerative clustering, in addition to providing an intuitive
% 	notion of inter-cluster distance (described below), also provides the ability
% 	to cluster without {pre-specifying} number of clusters.
% 
% %\para{Creating subreddit state clusters.} Using the topic and active
% %    user vectors generated in our previous step, we generated two clustering
% %    models -- one which clustered subreddit states by their topic vectors and
% %    another which clustered subreddit states by their active user vectors. In
% %    both cases, we used agglomerative (bottom-up) hierarchical ward-method
% %    clustering \cite{murtagh2014ward}. Agglomerative clustering starts off by
% %    treating each subreddit state individually and merging closest clusters
% %    together in a step by step process. Typically visualized as a dendrogram,
% %    clusters at higher levels are larger and more general while clusters at
% %    lower levels are much smaller and specific. Agglomerative clustering, in
% %    addition to providing an intuitive notion of inter-cluster distance
% %    (described below), also provides the ability to cluster without
% %    {pre-specifying} number of clusters.
% 
%   \para{Quantifying magnitude of evolution.} Given our hierarchical
%     cluster models based on topic and active user vectors, we used an intuitive
%     measure of similarity between two subreddit states. We quantified the
%     distance between subreddit states $s_i$ and $s_j$ as the \emph{height} of
%     the nearest common ancestor of $s_i$ and $s_j$. To compute this distance,
%     we performed a search for the nearest common ancestor of the input subreddit
%     states, computed the $\max$ of the number of nodes between this parent and
%     each of the subreddit states being compared (\ie $s_i$ and $s_j$).
%     Therefore, if the distance between the subreddit states associated with two
%     consecutive months of a subreddit is high, it is indicative that the (topic
%     or active user) vectors associated with the newer subreddit states are much
%     more similar to other subreddits than its own previous state. This is
%     indicative of topical or user base evolution towards other subreddits. We
%     expect that the evolutionary distance between consecutive months of
%     a subreddit will be one or two (\ie nearest parent is at distance one or
%     two from each state) in the event of convergence.
% 
% %   \para{Measuring nature of evolution.} In addition to quantifying the
% %     magnitude of evolution, we also present a method to measure the nature of
% %     change between consecutive subreddit states. For this, we relied on Latent
% %     Dirichlet Allocation (LDA) to assign topics associated with each cluster in
% %     our hierarchical cluster models. For each subreddit state, we obtained the
% %     text of its subreddit wiki. This text was then associated with all parents
% %     of this subreddit state in our hierarchical model. LDA was then performed
% %     on the text associated with every possible cluster in our model, therefore
% %     giving us a set of topics associated with every cluster. We also repeated
% %     this process with the comments associated with each cluster. These topics
% %     give us an insight into the topical direction in which subreddits are
% %     evolving. 
% %     
% % \Cref{fig:evolution:methods:dendro} shows a snippet of the dendrogram
% % associated with our topic vector based hierarchical cluster model. As leaves in
% % the dendrogram we have our subreddit states and with each parent in the tree
% % are topics extracted from the child subreddit wikis and comments using LDA.
% % This snippet shows how \subreddit{The\_Donald} moved from being most closely
% % associated with \subreddit{AskThe\_Donald} in late 2017 to being associated
% % most closely with the 2016-versions of now banned subreddits --
% % \subreddit{altright} and \subreddit{CringeAnarchy} in mid-2018. In this
% % example, we see that \subreddit{The\_Donald} has evolved a distance of
% % 3 between 08/2017 and 05/2018.
% % 
% % \Cref{fig:evolution:methods:dendro} shows a snippet of the dendrogram
% % associated with our topic vector based hierarchical cluster model. As leaves in
% % the dendrogram we have our subreddit states and with each parent in the tree
% % are topics extracted from the child subreddit wikis and comments using LDA.
% % This snippet shows how \subreddit{The\_Donald} moved from being most closely
% % associated with \subreddit{AskThe\_Donald} in late 2017 to being associated
% % most closely with the 2016-versions of now banned subreddits --
% % \subreddit{altright} and \subreddit{CringeAnarchy} in mid-2018. In this
% % example, we see that \subreddit{The\_Donald} has evolved a distance of
% % 3 between 08/2017 and 05/2018.
% 
\subsection{Results}\label{sec:evolution:results}

\subsubsection{Do subreddits converge to topic stability?}
\label{sec:evolution:results:topics}

\subsubsection{Do subreddits converge to active user base stability?}
\label{sec:evolution:results:users}

\subsubsection{Do subreddits in $\mathfrak{D}_I$ have different evolutionary
behaviors than subreddits in $\mathfrak{D}_A$?}
\label{sec:evolution:results:differences}

\subsubsection{Takeaway: Do subreddits need to be constantly monitored?}
\label{sec:evolution:results:takeaways}

% 
% We now quantify the magnitude of topical and active user base evolution for
% subreddits belonging to different datasets -- \ie $\mathfrak{D}_S$,
% $\mathfrak{D}_B$, and $\mathfrak{D}_H$. We specifically focus
% on measuring the average magnitude of evolution per month for different
% subreddits (\Cref{sec:evolution:results:distributions}) and how subreddits
% evolve as a function of their age (\Cref{sec:evolution:results:age}).
% {Based on these analyses, we expect to be able to test the hypothesis that
% subreddits do not always converge to user or topical stability
% (\Cref{sec:evolution:results:takeaway})}.

<<<<<<< HEAD
\begin{figure}[!h]
   \centering
        \includegraphics[width=.49\textwidth]{H1-cat-figs/topic-cluster-evolution.pdf}
        \includegraphics[width=.49\textwidth]{H1-cat-figs/topic-cluster-monthly.pdf}\\
        \includegraphics[width=.49\textwidth]{H1-cat-figs/topic-similarity-evolution.pdf}
        \includegraphics[width=.49\textwidth]{H1-cat-figs/topic-similarity-monthly.pdf}
	\hhnote{topic-evolution-cluster, topic-monthly-cluster, topic-evolution-similarity, topic-monthly-similarity}
  \label{fig:moderation:results:joining}
\end{figure}

\begin{figure}[!h]
   \centering
        \includegraphics[width=.49\textwidth]{H1-cat-figs/user-cluster-evolution.pdf}
        \includegraphics[width=.49\textwidth]{H1-cat-figs/user-cluster-monthly.pdf}\\
        \includegraphics[width=.49\textwidth]{H1-cat-figs/user-similarity-evolution.pdf}
        \includegraphics[width=.49\textwidth]{H1-cat-figs/user-similarity-monthly.pdf}
	\hhnote{user-evolution-cluster, user-monthly-cluster, user-evolution-similarity, user-monthly-similarity}
  \label{fig:moderation:results:joining}
\end{figure}


\begin{figure}[!h]
   %\centering
        \includegraphics[width=.49\textwidth]{H1-figs/plot-topic-evolution-relative.pdf}
        \includegraphics[width=.49\textwidth]{H1-figs/plot-topic-monthly-relative.pdf}\\
        \includegraphics[width=.49\textwidth]{H1-figs/plot-topic-evolution-similarity.pdf}
        \includegraphics[width=.49\textwidth]{H1-figs/plot-topic-monthly-similarity.pdf}
	\hhnote{top left: topic-evolution-relative, top right: topic-monthly-relative, topic-evolution-similarity, topic-monthly-similarity}
  \label{fig:moderation:results:joining}
\end{figure}



\begin{figure}[!h]
   %\centering
        \includegraphics[width=.49\textwidth]{H1-figs/plot-user-evolution-cluster.pdf}
        \includegraphics[width=.49\textwidth]{H1-figs/plot-user-monthly-cluster.pdf}\\
        \includegraphics[width=.49\textwidth]{H1-figs/plot-user-evolution-similarity.pdf}
        \includegraphics[width=.49\textwidth]{H1-figs/plot-user-monthly-similarity.pdf}
	\hhnote{user-evolution-cluster, user-monthly-cluster, user-evolution-similarity, user-monthly-similarity}
  \label{fig:moderation:results:joining}
\end{figure}

\subsubsection{How much do subreddit topics and active user bases evolve per
month?} \label{sec:evolution:results:distributions} 
We make the following observations from \Cref{tab:evolution:results} which
shows the distribution of the mean monthly magnitude of topical and active user
base evolution for subreddits in different categories.

\begin{table}
  \centering
  \small
  \begin{tabular}{p{.4in}p{1.2in}p{1.2in}}
    \toprule
    \textbf{Category} & \textbf{MTE} & \textbf{MUBE} \\
    \midrule
    $D_S$ & 4.4, 6.3, 8.0, 12.0, 24.8 & 3.2, 3.8, 4.2, 5.8, 12.0\\
    $D_H$ & 3.8, 8.8, 11.2, 12.7, 18.0 & 2.2, 2.4, 3.8, 4.2, 14.5\\
    $D_B$ & 3.4, 5.1, 6.5, 9.4, 21.2 & 2.3, 3.2, 4.2, 5.5, 16.1\\
    \bottomrule
  \end{tabular}
  \caption{The distribution of monthly topic evolution (\textbf{MTE}) and
  monthly user base evolution (\textbf{MUBE}) for different subreddit
  categories. The values represent the $1^{st}$, $25^{th}$, $50^{th}$,
  $75^{th}$, and $99^{th}$ percentile evolution distance values observed in our
  dataset.} 
  \vspace{-.25in}
  \label{tab:evolution:results}
\end{table}

  First, \emph{subreddits have a high average rate of evolution per month.}
    Looking at the average magnitude of topical and active user base
    evolution per month for different subreddit categories, we see that the
	median values for subreddits in different categories are between 6.5 \& 11.2
	for topic evolution and 3.8 \& 4.2 for user evolution. This is indicative that the average subreddit evolves at a high rate on average. For reference, an average value of 1 or 2 would
    indicate that the subreddit has not evolved since its conception. %We also
    %notice that, in general, the magnitude of evolution of user bases is lower
    %than of topics. 
  Second, \emph{the median magnitude of user evolution per month is consistent across
  subreddit categories, but the long tails vary.} We see that subreddit
  categories are not a discriminator when considering only the median monthly
  magnitudes of user evolution. However, we see that the distribution of these
  magnitudes varies by subreddit category. In particular, we see that
  subreddits in $\mathfrak{D}_B$ and $\mathfrak{D}_H$ are heavier
  weighted towards lower and higher average monthly magnitudes of user evolution --
  \ie subreddits in these groups are more likely to have extremely high or low
  average magnitudes of user evolution. This indicates that (1) some subreddits in
  $\mathfrak{D}_B$ and $\mathfrak{D}_H$ show more signs of being likely
  to converge to user base stability, but this is not a common
  case for any subreddit category and (2) different categories of subreddits
  might have different evolutionary patterns -- a promising insight for
  hypothesis H2 which aims to predict the subreddit category based on
  evolutionary patterns.

% In addition to measuring a subreddit's average magnitude of evolution, we are	
% also able to check the nature of subreddit evolution by observing the keywords
% of different subreddit states. We examine the \emph{most evolved} subreddit in each category
% to understand the nature of evolution in each case. There are highlighted in
% \Cref{tab:evolution:results:special}. Of particular interest are
% \subreddit{enoughsandersspam} and \subreddit{altright}. Studying the nature of
% evolution of \subreddit{enoughsandersspam} we see that the subreddit initially
% started as a subreddit to mock and harass supporters of US politician Bernie
% Sanders going as far as goading them into suicide and threatening rape
% \cite{ESS-threats}. This behavior resulted in its addition into
% $\mathfrak{D}_H$. However, we observe that the subreddit turned into
% a pro-Bernie Sanders community in late 2018 as a result of a moderator
% takeover \cite{ESS-takeover}. This resulted in an unusually high magnitude of
% active user base evolution. Similarly, we see that \subreddit{altright} emerged
% as a political movement in early 2016 and evolved into a white supremacist and
% anti-Semitic subreddit by early 2017. Our method identifies these
% subreddits as the most evolved and is able to hint at the nature of evolution,
% which serves as validation for the techniques and metrics in 
% \Cref{sec:evolution:methods}. 
=======
%  
% 
% \begin{figure}[!h]
%    %\centering
%         \includegraphics[width=.49\textwidth]{H1-figs/plot-topic-evolution-cluster.pdf}
%         \includegraphics[width=.49\textwidth]{H1-figs/plot-topic-monthly-cluster.pdf}\\
%         \includegraphics[width=.49\textwidth]{H1-figs/plot-topic-evolution-similarity.pdf}
%         \includegraphics[width=.49\textwidth]{H1-figs/plot-topic-monthly-similarity.pdf}
% 	\hhnote{topic-evolution-cluster, topic-monthly-cluster, topic-evolution-similarity, topic-monthly-similarity}
%   \label{fig:moderation:results:joining}
% \end{figure}
% 
% 
% 
% \begin{figure}[!h]
%    %\centering
%         \includegraphics[width=.49\textwidth]{H1-figs/plot-user-evolution-cluster.pdf}
%         \includegraphics[width=.49\textwidth]{H1-figs/plot-user-monthly-cluster.pdf}\\
%         \includegraphics[width=.49\textwidth]{H1-figs/plot-user-evolution-similarity.pdf}
%         \includegraphics[width=.49\textwidth]{H1-figs/plot-user-monthly-similarity.pdf}
% 	\hhnote{user-evolution-cluster, user-monthly-cluster, user-evolution-similarity, user-monthly-similarity}
%   \label{fig:moderation:results:joining}
% \end{figure}
% 
% \subsubsection{How much do subreddit topics and active user bases evolve per
% month?} \label{sec:evolution:results:distributions} 
% We make the following observations from \Cref{tab:evolution:results} which
% shows the distribution of the mean monthly magnitude of topical and active user
% base evolution for subreddits in different categories.
>>>>>>> ff9d5c57a9771f2ecbdaa75fc7650f97a1ca01a8
% 
% \begin{table}
%   \centering
%   \small
%   \begin{tabular}{p{.4in}p{1.2in}p{1.2in}}
%     \toprule
%     \textbf{Category} & \textbf{MTE} & \textbf{MUBE} \\
%     \midrule
%     $D_S$ & 4.4, 6.3, 8.0, 12.0, 24.8 & 3.2, 3.8, 4.2, 5.8, 12.0\\
%     $D_H$ & 3.8, 8.8, 11.2, 12.7, 18.0 & 2.2, 2.4, 3.8, 4.2, 14.5\\
%     $D_B$ & 3.4, 5.1, 6.5, 9.4, 21.2 & 2.3, 3.2, 4.2, 5.5, 16.1\\
%     \bottomrule
%   \end{tabular}
%   \caption{The distribution of monthly topic evolution (\textbf{MTE}) and
%   monthly user base evolution (\textbf{MUBE}) for different subreddit
%   categories. The values represent the $1^{st}$, $25^{th}$, $50^{th}$,
%   $75^{th}$, and $99^{th}$ percentile evolution distance values observed in our
%   dataset.} 
%   \vspace{-.25in}
%   \label{tab:evolution:results}
% \end{table}
% 
%   First, \emph{subreddits have a high average rate of evolution per month.}
%     Looking at the average magnitude of topical and active user base
%     evolution per month for different subreddit categories, we see that the
% 	median values for subreddits in different categories are between 6.5 \& 11.2
% 	for topic evolution and 3.8 \& 4.2 for user evolution. This is indicative that the average subreddit evolves at a high rate on average. For reference, an average value of 1 or 2 would
%     indicate that the subreddit has not evolved since its conception. %We also
%     %notice that, in general, the magnitude of evolution of user bases is lower
%     %than of topics. 
%   Second, \emph{the median magnitude of user evolution per month is consistent across
%   subreddit categories, but the long tails vary.} We see that subreddit
%   categories are not a discriminator when considering only the median monthly
%   magnitudes of user evolution. However, we see that the distribution of these
%   magnitudes varies by subreddit category. In particular, we see that
%   subreddits in $\mathfrak{D}_B$ and $\mathfrak{D}_H$ are heavier
%   weighted towards lower and higher average monthly magnitudes of user evolution --
%   \ie subreddits in these groups are more likely to have extremely high or low
%   average magnitudes of user evolution. This indicates that (1) some subreddits in
%   $\mathfrak{D}_B$ and $\mathfrak{D}_H$ show more signs of being likely
%   to converge to user base stability, but this is not a common
%   case for any subreddit category and (2) different categories of subreddits
%   might have different evolutionary patterns -- a promising insight for
%   hypothesis H2 which aims to predict the subreddit category based on
%   evolutionary patterns.
% 
% % In addition to measuring a subreddit's average magnitude of evolution, we are	
% % also able to check the nature of subreddit evolution by observing the keywords
% % of different subreddit states. We examine the \emph{most evolved} subreddit in each category
% % to understand the nature of evolution in each case. There are highlighted in
% % \Cref{tab:evolution:results:special}. Of particular interest are
% % \subreddit{enoughsandersspam} and \subreddit{altright}. Studying the nature of
% % evolution of \subreddit{enoughsandersspam} we see that the subreddit initially
% % started as a subreddit to mock and harass supporters of US politician Bernie
% % Sanders going as far as goading them into suicide and threatening rape
% % \cite{ESS-threats}. This behavior resulted in its addition into
% % $\mathfrak{D}_H$. However, we observe that the subreddit turned into
% % a pro-Bernie Sanders community in late 2018 as a result of a moderator
% % takeover \cite{ESS-takeover}. This resulted in an unusually high magnitude of
% % active user base evolution. Similarly, we see that \subreddit{altright} emerged
% % as a political movement in early 2016 and evolved into a white supremacist and
% % anti-Semitic subreddit by early 2017. Our method identifies these
% % subreddits as the most evolved and is able to hint at the nature of evolution,
% % which serves as validation for the techniques and metrics in 
% % \Cref{sec:evolution:methods}. 
% % 
% % \begin{table}
% %   \centering
% %   \small
% %   \begin{tabular}{p{1in}p{.25in}p{.25in}p{1.25in}}
% %     \toprule
% %     \textbf{Subreddit} & \textbf{AMM} & \textbf{LM} & \textbf{Nature of evolution}\\
% %     \midrule
% %     ($\mathfrak{D}_B$) \subreddit{altright}           & T:13.7 U:11.5 & T:31 U:17 & \red{right}, \red{support}, \red{vote}, \blue{jew}, \blue{white}, \blue{support} \\
% %       \midrule
% %     ($\mathfrak{D}_H$) \subreddit{enoughsandersspam}  & T:10.1 U:12.7 & T:50 U:53 & \red{bernie}, \red{the\_donald}, \red{spam}, \blue{hero}, \blue{obama}, \blue{original} \\
% %      \midrule
% %     ($\mathfrak{D}_S$) \subreddit{GalaxyNote7}        & T:30.7 U:22.0 & T:50 U:88 & \red{samsung}, \red{battery}, \red{nexus}, \blue{deals}, \blue{free}, \blue{blackfriday} \\
% %     \bottomrule
% %   \end{tabular}
% %   \caption{Subreddits with highest monthly evolution magnitudes in each
% %   category and the nature of their evolution. \textbf{AMM} is the average
% %   magnitude of evolution per month, \textbf{LM} is the magnitude of evolution
% %   over the entire lifetime of the subreddit, T and U denote the magnitudes of
% %   topic and active user base evolution, \red{Red} keywords represent
% %   topics associated with the start of the subreddit's lifetime, and \blue{Blue}
% %   keywords represent topics associated with the end of the subreddit's
% %   lifetime which is characterized by when the subreddit was banned or the end
% %   of our data collection (10/2018).}
% %   \label{tab:evolution:results:special}
% % \end{table}
% 
% % \begin{figure*}[th]
% %     \centering
% %     \begin{subfigure}{.485\textwidth} 
% %         \includegraphics[width=\textwidth]{evolution-figs/MeanContentBaseEvolution.png}
% %     \caption{Subreddit age vs magnitude of topic evolution.}
% %         \label{fig:evolution:results:convergetopic:lifetime}
% %     \end{subfigure}
% %     \begin{subfigure}{.485\textwidth} 
% %         \includegraphics[width=\textwidth]{evolution-figs/MeanUserBaseEvolution.png}
% %     \caption{Subreddit age vs magnitude of active user base evolution.}
% %         \label{fig:evolution:results:convergeuser:lifetime}
% %     \end{subfigure}
% % 
% %     \caption{Characteristics of topic and active user base evolution for
% %   subreddits in $\mathfrak{D}_A$, $\mathfrak{D}_B$, and $\mathfrak{D}_H$. 
% %   Figures (a) and (b) show the distribution of the mean magnitudes of
% %   topic and active user base evolution per month for subreddits in different
% %   categories. Figures (c) and (d) show the average magnitude of topic and
% %   active user base evolution as a function of subreddit age. The maximum lifetime
% %   of a subreddit is the time between the first post and last post in our
% %   datasets (our data collection ended on 10/2018). The `fraction of lifetime'
% %   is the fraction of this maximum lifetime. }
% %   \label{fig:evolution:results}
% % \end{figure*}
% % 
% 
% \subsubsection{How do subreddit topics and active user bases evolve as
% a function of subreddit age?} \label{sec:evolution:results:age}
% Our previous result shows that there is, on average, a significant magnitude
% of evolution per month for subreddits in all our categories. However, owing to
% the long tail distributions, we are unable to conclude that subreddits do not
% converge to topics or user bases. We now breakdown the magnitude of evolution
% by subreddit age. In the event of convergence, we expect to see that the
% magnitude of evolution drops to and stays at the minimum (1 or 2) after
% a certain point in the lifetime of a subreddit.
% \Cref{tab:evolution:results:age} shows the
% rate of evolution in different quarters of the subreddits existence. Q1 starts
% when the subreddit is created and Q4 ends on either May 2019 (the last month in
% our dataset) or on the date that the subreddit is banned. 
% We make the following conclusions from our results in
% \Cref{tab:evolution:results:age}.
% % \Cref{fig:evolution:results:convergetopic:lifetime} and
% % \Cref{fig:evolution:results:convergeuser:lifetime} show how subreddit topics 
% % and active user bases evolve as a function of their age. We can make the
% % following observation from these plots. 
% % 
% \begin{table}
%   \centering
%   \small
%   \begin{tabular}{p{.4in}p{1.3in}p{1.3in}}
%     \toprule
%     \textbf{Category} & \textbf{TE} & \textbf{UBE} \\
%     \midrule
%     $D_S$ & 8.4, 7.7, 9.8, 9.4 & 3.7, 2.7, 2.6, 2.9\\
%     $D_H$ & 12.0, 10.6, 11.3, 10.5 & 4.1, 3.5, 3.6, 3.9\\
%     $D_B$ & 8.3, 9.0, 10.6, 12.4 & 5.2, 4.0, 5.0, 4.8\\
%     \bottomrule
%   \end{tabular}
%   \caption{The distribution of mean topic (\textbf{TE}) and user base
%   evolution (\textbf{UBE}) for each subreddit category. The values
%   represent the average evolution observed during Q1, Q2, Q3, and Q4 of the
%   subreddit lifespan.}
%   \vspace{-.25in}
%   \label{tab:evolution:results:age}
% \end{table}
% %
%   \emph{Banned subreddits ($\mathfrak{D}_B$) show high magnitude evolutions
%   before being banned.} In
%   the case of $\mathfrak{D}_B$ we see that the magnitude of topic evolution has
%   a sharp increase in Q4 -- right before the subreddit is banned. We also
%   analyze the average net evolution over a lifetime for subreddits in each
%   category. Here again we find that subreddits in $\mathfrak{D}_B$ and
%   $\mathfrak{D}_H$ have significantly higher average magnitudes of topic
%   evolution (12.4 and 10.5, respectively) than other subreddits
%   ($\mathfrak{D}_S$ has a mean topic evolution magnitude of 9.4).  This is
%   indicative that subreddits which get banned or get labeled as hateful often
%   do not start with discussions or user bases which occur at the end of their
%   lifespan.
% 
% \subsubsection{Takeaway: Do subreddits converge to topical or user stability?}
% \label{sec:evolution:results:takeaway}
% Taken together, our results show that subreddits generally have a high average
% magnitude of topic and user base evolution (per month and over a lifetime) and
% this evolution, in most cases, is independent of the age of the subreddit.
% Therefore, \emph{we are unable to claim that subreddits always converge to
% topical or user stability -- \ie hypothesis H1 is valid}. This suggests that
% policies that involve verifying and applying moderation policies at the time of
% subreddit creation is not sufficient. Rather, the application of moderation
% policies need to be considered repeatedly over the course of the subreddit's
% lifetime. This suggests a very high attention cost for human administrators
% and moderators who need to (1) monitor how thousands of subreddits are evolving
% and (2) identify how and when to act to maintain community civility.
% 
% 
% % \textbf{user base analysis}
% % \textsc{\color{red}Present results showing how user bases evolve for different
% % communities. Our results have to show `evolution vs time' and `evolution vs
% % community size'. Analysis of all results need to consider: (1) the most evolved
% % communities, (2) the average community, (3) the least evolved communities, and
% % (4) our communities of interest. Break these results down by topics: Did the
% % most or least evolved communities have any common topics or themes?}a
% % 
% % Our first set of experiments uses user-vectors to look at user base stability.
% % Figure \ref{fig:Evolution} shows how user base evolves for the average reddit
% % community. We use data from all 3,000 subreddits in ($\mathfrak{D}_A$) and
% % measure the average distance between adjacent subreddit states on our
% % user-vector dendrogram. The results  show a clear monthly churn across
% % subreddits which suggests that the average subreddit's user base does not
% % converge. 
% % 
% % \begin{figure}[h!]
% % \includegraphics[width=\linewidth]{evolution-figs/ViolenUserBaseEvolution.png}
% % \includegraphics[width=\linewidth]{evolution-figs/DatasetDistributionUserEvolutionLinear.png}
% % \includegraphics[width=\linewidth]{evolution-figs/DistributionofMonthlyContentBaseEvolutionLinear.png}
% % % \includegraphics[width=\linewidth]{evolution-figs/DistancesDistributionperSubreddit.png}
% % \caption{user base evolution}
% % \label{fig:Evolution}
% % \end{figure}
% % 
% % We take a closer look at a few subreddits that have evolved more than others.
% % \textit{CrackStatus}, \textit{GrassrootsSelect} and \textit{enoughsandersspam}
% % etc for instance show a far bigger monthly user turn-over than others (Figure:
% % \ref{fig:Evolution}). \textit{enoughsandersspam} is an interesting case study
% % as it started out as an anti-bernie community and was taken over by pro-bernie
% % moderators from inside the administration\textsc{\color{red}[REFERENCE] whats
% % the source for evolved posters here, do we perform LDA? if so quote data}. The
% % user base of \textit{enoughsandersspam} has evolved from anti-bernie posters to
% % pro-bernie posters and explains the high monthly turn-over.
% % \textit{CrackStatus} is a community made exclusively for sharing news and
% % updates on cracks for video games, since the community discusses breakthrough
% % events happening in the field of cracks and piracy the frequency of such
% % discussion is sparse. The churn here can perhaps be explained by the
% % groundbreaking crack of the Denuvo DRM. The crack of this DRM led to influx of
% % new users in the subreddit therefore potentially explaining the evolution of
% % user base. \textit{GrassrootsSelect} on the other hand got shut-down and the
% % moderators moved the subreddit to \textit{Political\_Revolution}.
% % 
% % \textbf{user base stability over time}
% % We plot the mean distance between adjacent monthly subreddit states for all 4 Datasets in
% % order to explore user base stability over time(Figure \ref{fig:Evolution1}). Our results show that ($\mathfrak{D}_A$) has a constant churn of ~5 in evolution where as ($\mathfrak{D}_B$) and ($\mathfrak{D}_H$) on most occasions have a lower evolution. However the stability of the churn if looked closely shows that ($\mathfrak{D}_A$) doesn't radically change at any point except one which can be attributed as an anomaly. Where as ($\mathfrak{D}_B$) and ($\mathfrak{D}_H$) have several spikes in their evolution much higher than ($\mathfrak{D}_A$)'s evolution, that very strongly indicates that there are events in time that lead to an entire subreddit user base changing. 
% % % We
% % % show the evolution of some selected subreddits over the period of their
% % % lifetime and compare it with the average evolution over the whole of reddit. We
% % % observe that subreddits generally have higher churn in the initial months after
% % % they are created. \textit{The\_Donald} and \textit{altright} for example have
% % % a high magnitude of evolution in their initial period and while the communities
% % % continues to evolve over time, the initial churn slows down. Some subreddits
% % % however evolve significantly after several months \textit{uncensorednews} for
% % % instance has a high magnitude of evolution 14 months after its creation.
% % % Interestingly however, May 2017 sees a reddit-wide spike in evolution which can
% % % perhaps be attributed to an external global event. 
% % 
% % \begin{figure}[h!]
% % \includegraphics[width=\linewidth]{evolution-figs/MeanUserBaseEvolution.png}
% % \includegraphics[width=\linewidth]{evolution-figs/UserBaseEvolutionDistribution.png}
% % \caption{Evolution over time}
% % \label{fig:Evolution1}
% % \end{figure}
% % 
% % 
% % \textbf{Case Study: The\_Donald}
% % We take a closer look at the participants of \textit{The\_Donald} since its
% % creation in June 2016 (Figure \ref{fig:donald}). We use tSNE[REFERNECE] to
% % reduce dimensionality and plot the user-vectors of \textit{The\_Donald} and the
% % subreddits most similar to it. At inception \textit{The\_Donald} had more
% % participant overlap with groups closer to gaming and social media subreddits.
% % Over-time however, it evolved closer to the political and news subreddits. The
% % subreddit continues to evolve and ends up surrounded by subreddits such as
% % \textit{CringeAnarchy} and \textit{KotakuInAction} which we have labeled as
% % hateful subreddits. 
% % 
% % % TODO improve the graph
% % \begin{figure}[h!]
% % \includegraphics[width=\linewidth]{evolution-figs/TheDonaldEvolution.png}
% % \caption{The\_Donald evolution}
% % \label{fig:donald}
% % \end{figure}
% % 
% % \textbf{Content-base analysis}
% % In our next set of experiments, we use \textit{content-vectors} to look at
% % topical stability of subreddits. Using our content-vector based cluster, we
% % compute the average distances between adjacent subreddit states for our
% % complete subreddit dataset ($\mathfrak{D}_A$) (Figure: \ref{fig:content}). As
% % described previously, the topics that the community is actively discussing will
% % change as the discourse of the community changes, this gets reflected in the
% % higher distance between adjacent \textit{content-vectors}. The average
% % subreddit community does not seem to converge to a topical stability.%(prove
% % %this in a better way).
% % 
% % \begin{figure}[h!]
% % \includegraphics[width=\linewidth]{evolution-figs/ViolenContentBaseEvolution.png}
% % % \includegraphics[width=\linewidth]{evolution-figs/ContentBasedDistance.png}
% % % \includegraphics[width=\linewidth]{evolution-figs/BannedSubredditsContentBasedEvolution.png}
% % \caption{Content evolution}
% % \label{fig:content}
% % \end{figure
% % 
% % We take a closer look at a few selected subreddits that include banned,
% % quarantined or privatised subreddits and hateful subreddits. Banned subreddits
% % tend to have a higher topical instability compared to hateful subreddits.
% % Furthermore we can see that some subreddits that have topical instability such
% % as \textit{enoughsandersspam} also had user base instability. 
% % 
% % \textbf{Content Evolution over the life of a subreddit}
% % Our analysis over all subreddits in ($\mathfrak{D}_A$) shows that the average
% % subreddit content tends to evolve over time (Figure: \ref{evo-content} ). We
% % further analyze several subreddits by looking at the distance between their
% % initial states and their final states in our dataset. This helps us track the
% % magnitude of the drift in a subreddit's topics and content from its initial
% % topics. An good example of this is \textit{enoughsandersspam}, a subreddit
% % created for anti-bernie content which evolved into its opposite. We can see
% % this evolution reflect in both user-vectors and content-vectors. 
% % 
% % \begin{figure}[h!]
% % \includegraphics[width=\linewidth]{evolution-figs/MeanContentBaseEvolution.png}
% % \includegraphics[width=\linewidth]{evolution-figs/ContentBaseEvolutionDistribution.png}
% % \caption{Evolution over time}
% % \label{fig:evo-content}
% % \end{figure}
% % 
% % \begin{figure}[h!]
% % \includegraphics[width=\linewidth]{evolution-figs/MeanContentBaseEvolutionbyUsersChange.png}
% % \includegraphics[width=\linewidth]{evolution-figs/MeanContentBaseEvolutionbyActiveUsers.png}
% % \caption{Evolution over active users}
% % \label{fig:evo-content}
% % \end{figure}
% % 
% % 
% % 
% % \textsc{\color{red}Explain this figure?}\\
% % \includegraphics[width=\linewidth]{evolution-figs/SubredditEvolution.png}
% 

